Structural generalization is hard for sequence-to-sequence models

Sequence-to-sequence (seq2seq) models have been successful across many NLP tasks, including ones that require predicting linguistic structure. However, recent work on compositional generalization has shown that seq2seq models achieve very low accuracy in generalizing to linguistic structures that were not seen in training. We present new evidence that this is a general limitation of seq2seq models that is present not just in semantic parsing, but also in syntactic parsing and in text-to-text tasks, and that this limitation can often be overcome by neurosymbolic models that have linguistic knowledge built in. We further report on some experiments that give initial answers on the reasons for these limitations.

==> EMNLP 2022/figures/struct_gen_type.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{\columnwidth}
    \centering
    %\includegraphics[width=\textwidth]{figs/subj-obj-pp}
    \hbox{\tiny
      \input{figures/tree_to_subj_pp}
    }
    \caption{object PP to subject PP}\label{fig:structural-generalization:toSubjPP}
  \end{subfigure}
  
  \begin{subfigure}[b]{\columnwidth}
      \centering
      %\includegraphics[width=\textwidth]{figs/pp-recursion}
      \hbox{\tiny
        \input{figures/tree_pp_recursion}
      }
      \caption{PP recursion}\label{fig:structural-generalization:PPrecursion}
  \end{subfigure}
  \caption{Structural generalization in COGS.}
  \label{fig:structural-generalization}
\end{figure}

==> EMNLP 2022/figures/tree_pp_recursion.tex <==
% Ava saw the ball in the bowl on the table
% Ava saw the ball in the bowl on the table on the floor

%TODO: get spacing right (recursion trees more spread out in width and less in height?) --> see §2.4 Node positioning in manual
% some help:
%   [some long phrase,roof]  will draw a roof with 'some long phrase' at the bottom
%   fit=()(!1)(!2)  refers to nodes: the current one (), the first child (!1) and the second child (!2)   see 'relative nodes', page 8 in the forest doc
%   fit to=tree   fits to the whole subtree starting from the current node
%   s sep=8pt controls minimal distance between sibling subtrees (might want to decrease or strip)
%   inner sep=1  : compared to default, nodes have less surrounding 'space'
%   l=0, l sep=3   : control distance between levels (parent and children)
\begin{forest} for tree={l=0, l sep=3, s sep=6pt, inner sep=1}
[S 
  [NP [Ava]]
  [VP
    [V [saw]]
    [NP
      [NP [a ball,roof]]
      [PP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit=()(!1)(!2)]{};}
       [in]
       [NP
         [NP [a bowl,roof]]
         [PP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit=()(!1)(!2)]{};}
           [on]
           [NP [the table,roof]]
         ]
       ]
      ]
    ]
  ]
]
\end{forest}
\hspace{-1.5cm}
$\implies$

%\hspace{-1cm}
\begin{forest} for tree={l=0, l sep=3, s sep=6pt, inner sep=1}
[S 
  [NP [Ava]]
  [VP
    [V [saw]]
    [NP
      [NP [a ball,roof]]
      [PP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit=()(!1)(!2)]{};}
       [in]
       [NP
         [NP [a bowl,roof]]
         [PP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit=()(!1)(!2)]{};}
           [on]
           [NP 
             [NP [the table,roof]]
             [PP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit to=tree]{};}
               [on the floor,roof]
             ]
           ]
         ]
       ]
      ]
    ]
  ]
]
\end{forest}

==> EMNLP 2022/figures/tree_to_subj_pp.tex <==
% Noah ate the cake on the plate
% The cake on the table burned

% cf. https://linguistics.stackexchange.com/questions/34818/trying-to-add-labels-descriptions-and-boxes-to-syntax-tree-in-latex
\begin{forest} for tree={l=0, l sep=4, inner sep=1}
%sn edges/.style={for tree={parent anchor=south, child anchor=north}}, sn edges % edges merge at top
[S, s sep=1pt, 
  [NP [Noah]]
  [VP, s sep=10pt, 
    [V [ate]]
    [NP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit to=tree]{};}
      [NP [the cake,roof]]
      [PP [on the plate,roof]]
    ]
  ]
]
\end{forest}
\hspace{-5mm}
$\implies$

\begin{forest} for tree={l=0, l sep=4, inner sep=1}
[S, s sep=1pt,  
  [NP,tikz={\node [draw=black,fill=cyan!30, fill opacity=0.2,inner sep=0,fit to=tree]{};}
      [NP [the cake,roof]]
      [PP [on the table,roof]]
  ]
  [VP
    [V [burned]]
  ]
]
\end{forest}

==> EMNLP 2022/macros.tex <==
%% Additional packages and commands to be placed in the preamble

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{framed} %% debugging: boxes around figures to determine their size
%\usepackage{caption} % probably already loaded in emnlp2021.sty
% PW: is it allowed to descrease size between image and caption? \captionsetup[figure]{skip=5pt} % default is 10pt?
\usepackage{subcaption}  %% needed to have subfigures
\usepackage{tabularx}  %% X column for tables: automatic line breaks
\usepackage{booktabs}  %% nice tables: \toprule, \bottomrule, \midrule
\usepackage{multirow}  %% multirow in table with \multirow{number rows}{width}{text}
%\usepackage{tablefootnote}  %% for footnote to work in tables \tablefootnote[...]{...}
\usepackage{makecell}
% make siunitx and gb4e work together: https://tex.stackexchange.com/questions/364163/incompatibility-between-siunitx-and-gb4e
\makeatletter
\def\new@fontshape{}
\makeatother
\usepackage{siunitx} %% formatting numbers/units. used in appendix for detailed eval results formatting

\usepackage{xspace}  % \xspace command. add space after newcommand or don't (context-dependent) 
%% define font to be one point smaller (used for lform in typewriter) see https://tex.stackexchange.com/a/365025
%\makeatletter
%\newcommand{\oneptsmaller}[1]{%
%  \begingroup
%  \fontsize{\dimexpr\f@size pt-1pt}{\f@baselineskip}\selectfont
%  #1%
%  \endgroup
%}
%\makeatother

\usepackage{tikz}  %% drawing
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{calc, positioning}  % for bars in table
\usepackage{forest}  %% drawing linguistic trees: used for AM algebra figure: the AM term and the AM dep-tree and also for the PPrecursion/subjPP trees
\useforestlibrary{linguistics}
\forestapplylibrarydefaults{linguistics}

\usepackage{stmaryrd} %% denotation brackets (Lucia)

\usepackage[compress,sort,capitalise]{cleveref}  %% automatically insert type of reference: Figure/Table/Section...
  %% NB: should be placed after hyperref is loaded
\usepackage{hyperref}

\usepackage[inline]{enumitem}  %% customizing enumerations/lists: label=(\arabic*) or \Alph* ... or \roman*  , inliste list with starred version of normal lists: \begin{enumerate*}

\usepackage{gb4e}  % for linguistic examples \begin{exe} \ex example1 \ex example 2 \end{exe}
  %% ATTENTION: allows _ and ^ in ordinary text: can conflict with other commands/packages! 
  %% therefore use \noautomath directly after package loaded. see also https://tex.stackexchange.com/q/101300
\noautomath

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Defining own commands
\newcommand{\todo}[1]{\textcolor{red}{(\textbf{#1})}}
\newcommand{\todocite}{\todo{citation!}}
\newcommand{\sortof}[1]{`#1'}
\newcommand{\lform}[1]{\texttt{#1}}
%\newcommand{\lform}[1]{\oneptsmaller{\texttt{#1}}}
%\newcommand{\graphedge}[1]{\textsl{#1}}
\newcommand{\graphedge}[1]{`#1'}
\newcommand{\graphnode}[1]{`#1'}
\newcommand{\word}[1]{``#1''}
\newcommand{\phrase}[1]{``#1''}
\newcommand{\sentence}[1]{``#1''}

%\crefname{section}{sec.}{secs.} % see page 14 (sec 8.1.2) in the cleveref documentation
%\crefname{section}{tab.}{tabs.}
% make cleverref aware of examples and cite them with sourrounding parenthesis: see https://tex.stackexchange.com/a/318983
% if we can't use cleveref we could define a command \newcommand{\pref}[1]{(\ref{#1})} like suggested in https://tex.stackexchange.com/a/211871
\crefname{xnumi}{}{}
\creflabelformat{xnumi}{(#2#1#3)}
\crefrangeformat{xnumi}{(#3#1#4)--(#5#2#6)}

% tikz node and edge style for graphs
%  normal node
\tikzstyle{nnode} = [ellipse, text centered, draw=black, inner sep=2pt] %, outer sep=0pt
%  determiner node
\tikzstyle{dnode} = [rectangle, rounded corners, text centered, draw=black] % minimum width=3cm, minimum height=1cm, , fill=red!30
\tikzstyle{arrow} = [thick,->,>=stealth]

% for reference: the color values used in lindeman-etal-2019-compositional
%\colorlet{colorwant}{green!30}
%\colorlet{colorboy}{brown!10!yellow!60}
%\colorlet{colorthe}{blue!30}
%\colorlet{colorgo}{red!30}
% new colors should help colorblind, but actually more an excuse, just wanted to experiment with colors ;) - pw
\definecolor{colorwant}{HTML}{ABBEF1} % lighter blue tone
\definecolor{colorgo}{HTML}{DE8BB3} % red-pink tone
\definecolor{colorthe}{HTML}{F1AD83} % light orange tone
\definecolor{colorboy}{HTML}{FFE19D} % light yellow tone

% AM algebra things: %%%%%%%%%%%
\newcommand{\sources}{\ensuremath{\mathcal{S}}}
\newcommand{\tp}[1]{\ensuremath{\tau(#1)}}   % type variable
\newcommand{\type}[1]{\ensuremath{[#1]}}

\newcommand{\app}[1]{\text{\textsc{App}}\ensuremath{_{#1}}\xspace}
\newcommand{\modify}[1]{\text{\textsc{mod}}\ensuremath{_{#1}}\xspace}
\newcommand{\lignore}{\text{\textsc{ignore}}}
\newcommand{\of}[1]{\left(#1\right)}

% source
\newcommand{\src}[1]{\text{\textsc{#1}}\xspace} % source name 
%\newcommand{\obj}[1][]{\text{\src{o}}\ensuremath{_{#1}}} % object sources. \obj or \obj[i]
\newcommand{\subj}{\text{\src{s}}} % subject source, just \subj
% \newcommand{\op}[1][i]{\text{\src{op}}\ensuremath{_{#1}}} % op sources \op[i]
\newcommand{\rt}{\src{rt}} % root source
% with color red:
\newcommand{\srcr}[1]{\textcolor{red}{\src{#1}}} % source name 

\newcommand{\G}[1]{\ensuremath{G_{\text{#1}}}} % naming graphs


%% Colored bars as background in tables using \asbar
% this is based on TeX code found on arXiv for the Ontanon et al paper: https://arxiv.org/abs/2108.04378
\pgfdeclarelayer{background}
\pgfdeclarelayer{main}
\pgfsetlayers{background,main}
\newcommand*{\minWidth}{25}  % controls size of total box
\newcommand*{\maxValue}{100}
\newcommand{\makeBar}[3]{%
  \tikz[baseline]{
    \node[anchor=base,text width=\minWidth,align=#2,inner sep=0pt,inner xsep=4pt,outer sep=0pt] (n) {\strut{\hfill#1}};  % ,draw=black % \hfill makes numbers right-aligned
    \begin{pgfonlayer}{background}
        {
       \edef\color{#3}
       \pgfmathparse{abs(#1/\maxValue)}
       \edef\contents{{\pgfmathresult}}
       \fill[font=\boldmath,color=\color] (n.north west) rectangle ($(n.south west)!{{\contents}}!(n.south east)$);  %% that's the box for the actual percentage
       \fill[font=\boldmath,color=cyan!10] ($(n.north west)!{{\contents}}!(n.north east)$) rectangle (n.south east);  % that's the box for the rest
       }
    \end{pgfonlayer}
  }
}
\newcommand{\asbar}[1]{\makeBar{#1}{center}{cyan!25}}
\newcommand{\stderr}[1]{\tiny$\pm$#1}
% \newcommand{\stderr}[1]{\footnotesize{$\pm$#1}}

% Class names 'Lexicalized'/'ObjProper'/'Structural'
\newcommand{\genclass}[1]{\textsc{#1}\xspace} % 
\newcommand{\lexg}{\genclass{Lex}}
\newcommand{\propg}{\genclass{Prop}}
\newcommand{\structg}{\genclass{Struct}}

% how should we call AM parser models with and without BERT?
% NOTE: don't forget to change it in the recursion depth plot too!!!
\newcommand{\amBert}{AM+B} %AM+BERT  
\newcommand{\amToken}{AM} %AM-BERT aka AM Token
\newcommand{\dist}{dist\xspace} %with distance info added

\newcommand{\oldNumber}[1]{\textcolor{black!40}{#1}}

% Author comments
\usepackage{color}
\newcommand\bmmax{0} % magic to avoid 'too many math alphabets' error
\usepackage{bm}
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{mdgreen}{rgb}{0.05,0.6,0.05}
\definecolor{mdblue}{rgb}{0,0,0.7}
\definecolor{dkblue}{rgb}{0,0,0.5}
\definecolor{dkgray}{rgb}{0.3,0.3,0.3}
\definecolor{slate}{rgb}{0.25,0.25,0.4}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{ltgray}{rgb}{0.7,0.7,0.7}
\definecolor{purple}{rgb}{0.7,0,1.0}
\definecolor{lavender}{rgb}{0.65,0.55,1.0}
\definecolor{brown}{rgb}{0.6,0.2,0.2}

\newcommand{\ensuretext}[1]{#1}
\newcommand{\ldmarker}{\ensuretext{\textcolor{purple}{\ensuremath{^{\textsc{L}}_{\textsc{D}}}}}}
\newcommand{\pwmarker}{\ensuretext{\textcolor{magenta}{\ensuremath{^{\textsc{P}}_{\textsc{W}}}}}}
\newcommand{\yymarker}{\ensuretext{\textcolor{mdgreen}{\ensuremath{^{\textsc{Y}}_{\textsc{Y}}}}}}
\newcommand{\jgmarker}{\ensuretext{\textcolor{orange}{\ensuremath{^{\textsc{J}}_{\textsc{G}}}}}}
\newcommand{\akmarker}{\ensuretext{\textcolor{blue}{\ensuremath{^{\textsc{A}}_{\textsc{K}}}}}}
\newcommand{\codemarker}{\ensuretext{\textcolor{brown}{CODE}}}


\newcommand{\arkcomment}[3]{\ensuretext{\textcolor{#3}{[#1 #2]}}}
%\renewcommand{\arkcomment}[3]{}
%\renewcommand{\todo}[1]{}
\newcommand{\ld}[1]{\arkcomment{\ldmarker}{#1}{purple}}
\newcommand{\pw}[1]{\arkcomment{\pwmarker}{#1}{magenta}}
\newcommand{\yy}[1]{\arkcomment{\yymarker}{#1}{mdgreen}}
\newcommand{\jg}[1]{\arkcomment{\jgmarker}{#1}{orange}}
\newcommand{\ak}[1]{\arkcomment{\akmarker}{#1}{blue}}
\newcommand{\code}[1]{}%\arkcomment{\codemarker}{#1}{brown}}% marks discrepancies between text and code. Change this to {} for print version



\newcommand{\linf}{structure-aware}
\newcommand{\Linf}{Structure-aware}

\newcommand{\cogsqa}{QA-COGS}
\newcommand{\cogsqabase}{\cogsqa -base}
\newcommand{\cogsqacc}{\cogsqa -disamb}

\newcommand{\syncogs}{Syntax-COGS}
\newcommand{\poscogs}{POS-COGS}


\renewcommand{\paragraph}[1]{\textbf{#1}}

==> EMNLP 2022/sections/Background.tex <==



\section{Structural generalization in COGS}\label{sec:background}

% In this paper, we focus on structural generalization in COGS and in corpora that are derived from COGS. We will thus begin by introducing the COGS corpus.
\input{figures/struct_gen_type}


COGS \cite{kim-linzen-2020-cogs} is a synthetic semantic parsing
dataset in which English sentences must be mapped to logic-based
meaning representations (see Fig.~\ref{fig:cogssamples} for some examples). It distinguishes 21 \emph{generalization
  types}, each of which requires generalizing from training instances
to test instances in a particular systematic and
linguistically-informed way. COGS was designed to measure \emph{compositional generalization}, the ability of a semantic parser to assign correct meaning representations to out-of-distribution sentences. Unlike SCAN and CFQ, it includes generalization types with unbounded recursion and separates them cleanly from other generalization types, both of which are crucial for the experiments reported here.

Most generalization types in COGS are \emph{lexical}: they recombine known grammatical structures with words that were not observed in these particular
structures in training.  An example is the generalization type
``subject to object'' (\cref{fig:cogssamples}a), in which a
 noun (``hedgehog'') is only seen as a subject in training,
whereas it is only used as on object at test time. The syntactic structure at test time was already observed in training; only the words change.


  % Note that the syntactic structure at generalization time (e.g.\ that
  % of a transitive sentence) was already observed in training. On the
  % semantics side, the meaning representations are identical, except
  % for replacing some constants and quantifiers and renaming some
  % variables.
  % Thus, lexical generalization in COGS amounts to
  % learning how to fill fixed templates.

By contrast, \emph{structural generalization} involves generalizing to
linguistic structures that were not seen in training (cf.\
\cref{fig:cogssamples}b,c). Examples are the generalization types ``PP
recursion'', where training instances contain prepositional phrases of
depth up to two and generalization instances have PPs of depth 3--12;
and ``object PP to subject PP'', where PPs modify only objects in
training and only subjects at test time. These structural changes are
illustrated in 
\cref{fig:structural-generalization}.
%illustrates, structural
%generalization types ask the semantic parser to assign meaning to
%sentences of syntactic structures that were not seen in
%training.% Recursive types can be extended unboundedly.

Structural generalization requires learning about recursion and compositionality, and is thus a more thorough test of human-like language use, whereas lexical generalization amounts to smart template filling. In this paper, we investigate how well structural generalization can be solved by different classes of model architectures: \textit{seq2seq models} and \textit{\linf\ models}. We define a model as ``\linf''
if it is explicitly designed to encode linguistic knowledge beyond the fact that sentences are sequences of tokens. This captures a large class of models that can be as ``deep'' as a compositional semantic parser or as ``shallow'' as a POS tagger that requires that each input token gets exactly one POS tag.

% models as any models that are designed with task-specific architectures and thus can be aware of linguistic knowledge. Compared with seq2seq models which can generate arbitrary outputs, \linf\ models are explicitly constrained with linguistic knowledge and we expect they can generalize better than seq2seq models on our tasks.   
%   This distinction is borne out in model
%   performance (\cref{subsec:first:experiments}): while lexical
%   generalization can be handled by many neural architectures,
%   structural generalization requires parsing architectures aware of
%   complex sentence structure.




==> EMNLP 2022/sections/Conclusion.tex <==
\section{Conclusion}
We have presented evidence that structural generalization is hard for seq2seq models, both on semantic and syntactic parsing (COGS and \syncogs) and on some text-to-text tasks (\cogsqacc). In many of these cases, \linf\ models generalize successfully where seq2seq models struggle. Unlike earlier work, we have shown that this effect persists when the seq2seq models can be pretrained.

We have then presented a number of experiments to help pinpoint the cause of this limitation. We found that the BART encoder still provides structural information, but the decoder does not use it to generalize -- both in the parsing tasks and in the probing tasks on the original splits, and not even when the input is enriched with syntactic information. We further found that when the decoder's task is simple enough, as in \cogsqabase, seq2seq models learn to generalize structurally as well as \linf\ models. In improving the ability of seq2seq models to generalize structurally, it seems promising to focus on the decoder, especially by including \linf\ elements.


\section{Limitations} 
Our experiments are limited to a synthetic corpus (COGS) and its derivatives. While it seems plausible to us to justify negative results like ours with a synthetic corpus, it must be recognized that the distribution of language in COGS is not the same as in English as a whole, which might undermine the ability of both seq2seq and \linf\ models to learn to generalize.

Furthermore, claims about a whole class of models (seq2seq) can only be supported, never completely proved, through empirical experiments on a finite set of representatives. Nonetheless, we think that this paper has considered a sufficiently wide range of models and tasks to make careful statements about seq2seq models as a class.

\section*{Acknowledgements}
We are indebted to Lucia Donatelli and Pia Weißenhorn for fruitful discussions, and to Najoung Kim for providing the code for generating COGS.
This work was supported by the Deutsche Forschungsgemeinschaft (DFG) through the project KO 2916/2-2. 


==> EMNLP 2022/sections/Experiment.tex <==
\section{Experiments}

\subsection{setup}
\paragraph{QA setup} \label{subsec:seq2seq:setup}
We train BART as our model on QA-COGS.  To apply BART for the question answering task, we directly fine-tune the pretrained \textit{bart-base} model on it with the corresponding tokenizer. During fine-tuning, the model takes as input the concatenation of context and question strings and outputs the answer.

We also had another model named BART-QA for comparison. BART-QA simply applies two multi-layer perceptrons over the hidden states from BART to determine the start and end index of a span in the context. The selected span is used as the predicted answer. 

% \paragraph{\textcolor{red}{which other models should we use for experiments}}If the focus of the whole story is  \textit{seq2seq models fail on compgen}, we should also use LSTM (with copy mechanism) and perhaps GRU. If the focus is \textit{compgen on text-to-text generation tasks}, we should also give some space for extract question answering model.

\subsection{results}

Table \ref{tab:selected_gentype_eval} shows the results of our models on QA-COGS. We can observe that seq2seq models solve the predicate classification task, but still struggle on argument identification and relation tasks. We thus focus on discussing these results on these two tasks.

% \input{tables/qa_detailed_results}

\paragraph{Lexical Generalization} We first look at argument relation task. Clearly, seq2seq solves most lexical generalization types except for \textit{prim\_to\_subj\_proper}, \textit{prim\_to\_obj\_proper} and \textit{prim\_to\_inf\_arg}. Looking into the output of the model, we find that errors for such primitive generalization types all come from the inability to copy the primitive as seen below. 
\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{Noah imagined that Emma supported that Paula wanted to dance .}
    
    \textbf{Question} \textit{Who did Noah imagine that Emma support that want to dance ?}
    
    \textbf{Gold} \textit{Paula}
    
    \textbf{Pred} \textit{Paula Paula}
    
    }
}
\end{center}

Note that a primitive in original COGS is only annotated as either its word form or a lambda expression, so we cannot generate question-answer pairs for primitives in the train set. This means that such primitives (e.g. \textit{Paula} and \textit{crawl}) are out-of-vocabulary tokens for our model. We consider such errors are mainly due to the instability of fine-tuning our pretrained seq2seq models. \textcolor{red}{We should also use seq2seq with copy mechanism to get a better picture here.} However, another question exists: why the model can meanwhile solve the common noun cases (e.g. \textit{prim\_to\_obj\_common})? Does BART have some internal weakness for proper nouns? We currently do not have a clear answer for this. \textcolor{red}{ T5 does not have this issue so maybe this paragraph does not make much sense and we can just say it's the internal weakness of BART. Of course we can replace \textit{Paula} in the generalization set with other proper nouns to confirm this assumption.} T5 and extractive model perform well on this type. 

Now look at the argument relation task. Both extractive and seq2seq models cannot fully solve \textit{prim\_to\_obj\_proper}. However, we notice that for the same sentence, the two models make different types of errors as seen in the example below. \todo{Maybe I should add primitive word into the train set or try T5 on this task. This discussion does not make much sense to myself.} If extractive model cannot recognize Paula as a theme, how could it solve the argument relation task? Noticing that in relation task the question will become \textit{What did Emma sell the girl?}, we consider the extractive model simply learns to select the span not occurring in the question string. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{Emma sold the girl Paula .}
    
    \textbf{Question} \textit{What is the theme of sell ?}
    
    \textbf{Gold} \textit{Paula}
    
    \textbf{BART Pred} \textit{the girl}
    
    \textbf{BART-QA Pred} \textit{the girl Paula}
    
    }
}
\end{center}

\paragraph{obj\_pp\_to\_subj\_pp} Still we first look at the argument relation task. Different from the COGS result, seq2seq models performs well on \textit{obj\_pp\_to\_subj\_pp} type. Does this mean seq2seq model learns to combine PP structure with any nouns? Notice that to give the correct answer in the example below, the model can simply copy the context string on the left of the predicate word (e.g. screamed). Thus, this type is not enough to evaluate the ability to learn structure. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{ The baby on a tray in the house screamed .}
    
    \textbf{Question} \textit{ Who screamed ?}
    
    \textbf{Gold} \textit{ the baby on a tray in the house}
    
    \textbf{Pred} \textit{ the baby on a tray in the house}
    
    }
}
\end{center}

On the other hand, both seq2seq and extractive models does not solve this type in argument identification task. We find the main reason for this error is that both models possibly ignore the prepositional phrase modifying the subject as seen below. \todo{This actually could be counted as correct, though I do not know if this makes much sense.}
\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{A donkey in the room sold Ella a donut .}
    
    \textbf{Question} \textit{What is the agent of sell ?}
    
    \textbf{Gold} \textit{a donkey in the room}
    
    \textbf{BART Pred} \textit{a donkey}
    
    \textbf{BART-QA Pred} \textit{a donkey}
    
    \textbf{Question} \textit{What is the theme of sell ?}
    
    \textbf{Gold} \textit{a donut}
    
    \textbf{BART Pred} \textit{a donut in the room}
    
    \textbf{BART-QA Pred} \textit{a donut}
    
    }
}
\end{center}

\paragraph{recursion types} For CP and PP recursion types on relation task, our result is consistent with the pattern in semantic parsing. An error example for CP recursion is listed below. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{ Aiden liked that Liam liked that Avery appreciated that the dog expected that a cat liked that Emma appreciated that a donut was loved .}
    
    \textbf{Question} \textit{ What did Aiden like that Liam like?}
    
    \textbf{Gold} \textit{ that Avery appreciated that the dog expected that a cat liked that Emma appreciated that a donut was loved}
    
    \textbf{Pred} \textit{ that Avery appreciated that the dog expected that a cat liked that a cat liked that a cat.....}
    
    }
}
\end{center}

Again, such questions can be solved by simply generating the context string on the left of \textit{...that Liam like}. However, our result indicates that the seq2seq model does not even learn this simple heuristic. We also plot the result of our model with regard to answer recursions and context recursions for CP\_recursion typed sentences in Fig \ref{fig:qa_depth}. We can observe that for all depths of contexts, the performance always decreases as the answer depth grows. This is consistent with previous findings that seq2seq struggles on generating longer sequence than it sees during training, since our train set only contains sentences with at most 2 CP recursions. Another observation is that, for the same answer depth, larger context depth gives lower performance. However, this does not hold for answer depth 1 and 2, where the model performs well on cd=11-12 but worse on cd=6-8. We do not a good explanation about this for now. 
 
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/qa_recursion_depth.pdf}
    \caption{Exact match accuracy of BART on CP recursion typed questions. Answer depth denotes the number of CP recursions in the answer and \textit{cd} denotes the number of CP recursions in the context. \textcolor{red}{Need to make this figure easier to read.}}
    \label{fig:qa_depth}
\end{figure}

For identification task, seq2seq still struggle on both types. Interestingly, extractive models could solve \textit{pp\_recursion} but cannot solve \textit{cp\_recursion}. An example is shown below. We currently do not know why this happens.

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{A girl valued that Samuel admired that a monkey liked that Luna liked that Oliver respected that Savannah hoped that a penguin noticed that Emma noticed that the lawyer noticed that a cake grew .}
    
    \textbf{Question} \textit{ What is the agent of respect ?}
    
    \textbf{Gold} \textit{Oliver}
    
    \textbf{BART-QA Pred} \textit{Samuel}
    
    }
}
\end{center}

% \input{tables/qa_prim_error_examples}

% \paragraph{\textcolor{red}{Are we learning heuristics rather than compositionality?}} I feel that what I can say in this section is very shallow and I am now very worried that our model learns a lot of heuristics rather than compositionality to solve QA-COGS. Most examples in Table \ref{tab:qacogssamples} can be solved by some simple heuristics (e.g. output part of the context string which does not appear in the question string) rather than compositional generalization. If model only learns such heuristics, then this corpus really does not make any sense. 

% For example, for \textit{unacc\_to\_transitive} generalization type, we only have one sample in the train set below:

% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ Julian shattered .}
    
%     \textbf{Question} \textit{ What was shattered ?}
    
%     \textbf{Gold} \textit{ Julian}
    
%     \textbf{MR} \textit{ shatter . theme ( x \_ 1 , Julian )}
    
%     }
% }
% \end{center}

% % \textit{Context: Julian shattered .}

% % \textit{Q: What was shattered ?}

% % \textit{gold: Julian}

% % \textit{MR:  shatter . theme ( x \_ 1 , Julian )}

% and then in the generalization set we have:

% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The cat shattered the cake .}
    
%     \textbf{Question} \textit{ What did the cat shatter ?}
    
%     \textbf{Gold} \textit{ the cake}
    
%     \textbf{MR} \textit{ * cat ( x \_ 1 ) ; * cake ( x \_ 4 ) ; shatter . agent ( x \_ 2 , x \_ 1 ) AND shatter . theme ( x \_ 2 , x \_ 4 )}
    
%     }
% }
% \end{center}

% In semantic parsing task this makes sense, but in QA-COGS this task becomes too simple and can be solved by not using compositionality. This issue almost holds for all lexical generalization types, so we really should address this. 

% Another question I am considering is to ask different questions. Remember that the motivation of bAbI is to evaluate different reading comprehension abilities of neural models through a lot of toy tasks. (Our corpus is actually the task 5 \href{https://arxiv.org/pdf/1502.05698.pdf}{here}). As I mentioned in section \ref{sec:overview}, we can similarly split COGS into multiple tasks and evaluate them independently. As I can imagine, to solve COGS we need at least four abilities: 1) the ability to recognize the frame of a predicate 2) the ability to find the argument for a predicate 3) the ability to differentiate common nouns and proper nouns 4) the ability to count the index of a token. Our current corpus only tests the ability (2), so can we also test other abilities by asking new questions? 

% For example, to test ability (1), we can have questions like below:
% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The cat shattered the cake .}
    
%     \textbf{Question} \textit{ Which arguments does \textit{shatter} take ?}
    
%     \textbf{Gold} \textit{ agent theme}
    
%     }
% }
% \end{center}
% Such questions may also give us a better picture about whether our model learns heuristic or compositionality. 

% To test the ability (3), we may have:
% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The captain ate.}
    
%     \textbf{Question} \textit{ What is the index of \textit{captain}?}
    
%     \textbf{Gold} \textit{ 1}
    
%     }
% }
% \end{center}
% If the model cannot even solve this task for recursion types in the generalization set, it indicates that the failures of seq2seq on recursion generalization in COGS may be due to the counting inability.

==> EMNLP 2022/sections/Introduction.tex <==
% !TeX root = emnlp2022.tex

\section{Introduction} \label{sec:intro}

Humans are able to understand and produce linguistic structures they have never observed before \citep{chomsky-1957-syntactic,fodor-pylyshyn-1988-connectionism,fodor-lepore-2002-compositionality}. From limited, finite observations, they generalize at an early age to an infinite variety of novel structures using recursion. They can also assign meaning to these, using the Principle of Compositionality. 
This ability to generalize to unseen structures is important for NLP systems in low-resource settings, such as underresourced languages or projects with a limited annotation budget, where a user can easily use structures that had no annotations in training.

Over the past few years, large pretrained sequence-to-sequence (seq2seq) models, such as BART \citep{lewis-etal-2020-bart-acl} and T5 \citep{raffel-etal-2020-t5}, have brought tremendous progress to many NLP tasks. This includes linguistically complex tasks such as broad-coverage semantic parsing, where e.g.\ a lightly modified BART set a new state of the art on AMR parsing \citep{bevilacqua-etal-2021-one}. However, there have been some concerns that seq2seq models may have difficulties with \emph{compositional generalization}, a class of tasks in semantic parsing where the training data is structurally impoverished in comparison to the test data \citep{lake-baroni-2018-generalization,keysers-etal-2020-measuring}. We focus on the COGS dataset of \citet{kim-linzen-2020-cogs}
%, a synthetic semantic parsing dataset, 
because some of its generalization types specifically target \emph{structural generalization}, i.e.\ the ability to generalize to unseen structures.

In this paper, we make two contributions. First, we offer evidence that structural generalization is systematically hard for seq2seq models. On the semantic parsing task of COGS, seq2seq models don't fail on compositional generalization as a whole, but specifically on the three COGS generalization types that require generalizing to unseen linguistic structures, achieving accuracies below 10\%. This is true both for BART and T5 and for seq2seq models that were specifically developed for COGS. What's more, BART and T5 fail similarly on syntax and even POS tagging variants of COGS (introduced in this paper), indicating that they do not only struggle with \emph{compositional} generalization in semantics, but with \emph{structural} generalization more generally. \Linf\ models, such as the compositional semantic parsers of \citet{liu-etal-2021-learning} and \citet{weissenhorn22starsem} and the Neural Berkeley Parser \citep{kitaev-klein-2018-constituency}, achieve perfect accuracy on these tasks.

% AK moved it way up here to make sure it goes on page 2.
\input{tables/cogs_examples}


Second, we conduct a series of experiments to investigate what makes structural generalization so hard for seq2seq models. It is not because the encoder loses structurally relevant information: One can train a probe to predict COGS syntax from BART encodings, in line with earlier work \citep{hewitt-manning-2019-structural,tenney-etal-2019-bert}; but the decoder does not learn to use it for structural generalization. We find further that the decoder does not even learn to generalize semantically when the input is enriched with syntactic structure. Finally, it is not merely because the COGS tasks require the mapping of language into symbolic representations. We introduce a new text-to-text variant of COGS called \emph{\cogsqa}, where  questions about COGS sentences must be answered in English. We find that T5 performs well on structural generalization with the original COGS sentences, but all models still struggle with a harder text-to-text task involving structural disambiguation. %This suggests a deep limitation of sequence decoders for structural generalization. 

The code\footnote{\url{https://github.com/coli-saar/Seq2seq-on-COGS}} and datasets\footnote{\url{https://github.com/coli-saar/Syntax-COGS}} are available online.



==> EMNLP 2022/sections/New_generalization_types.tex <==

\section{Structural generalization without length generalization}
% \todo{Maybe this section could just be a subsection of QA-COGS. I do not think we say more beyond \textit{seq2seq and extractive models still fail on struct generaliation on QA.}}
We have seen the generalization set of QA-COGS has some limitations: the Obj to Subj PP type tests shallow compositionality while recursion types only tests length generalization ability. It is still unclear whether structural generalization is difficult or not when disentangled from length generalization. To explore this question, we create two new QA  datasets named \textit{cc\_cp} and\textit{rc\_pp} and observe model behaviours on these new datasets.

We start by introducing \textit{cc\_cp} corpus. The idea of this dataset is to test whether the model can generalize to unseen combination of the coordination structure(\textit{cc}) and the complement clause(\textit{cp}). An example is shown in the \textit{cc\_cp} row in Table \ref{tab:coordination_cp_example}. During training, the model sees context sentences with either a coordination structure (e.g. \textit{sleeps and jogs}) or a complement clause (e.g.  \textit{liked that Noah discovers a boy}), but never observes their combination in one context sentence. In the generalization set, we combine these two structures into one context sentence(e.g. \textit{liked that Noah discovers a boy and jogged}) and ask the question \textit{What did Oliver like?}. To answer this correctly, the model needs to be aware that verb tenses inside the coordination structure should be the same, and thus verb tenses determine whether the last verb(e.g. jog) should be coordinated with the verb inside the complement clause(e.g. discover) or outside the complement clause(e.g. like). 

Similarly, we test the combination of the relative clause structure(\textit{rc}) and the prepositional phrase structure(\textit{pp}) in \textit{rc\_pp}. The example is shown in the \textit{rc\_pp} row in Table \ref{tab:coordination_cp_example}. In this dataset we make the model learn \textit{rc}(e.g. \textit{boxes that were sketched}) and \textit{pp}(e.g. \textit{boxes in the house}) structure separately, and test their combination(e.g. \textit{boxes in the house that was sketched}) with the question \textit{What was sketched?}. To answer this correctly, the model needs to learn whether \textit{rc} modifies the noun inside \textit{pp} or outside \textit{pp} based on its verb form(e.g. \textit{was/were}).

Now we describe how we create such datasets in practice. For \textit{cc\_cp}, the train set consists of \textit{cp} sentences and \textit{cc} sentences. For \textit{cp} sentences, we directly copied from the original QA-COGS train set. For \textit{cc} sentences, we randomly sample 2000 sentences(without \textit{cp} structure) from  original QA-COGS train set and adding an unergative verb to the sampled sentences. The generalization set is then generated with a hand-written heuristic based on each \textit{cp} sentence in the train set. As shown in Figure \ref{fig:struct_example}, each \textit{cp} sentence in the train set will result in 4 sentences in generalization set. For\textit{rc\_pp}, the train set consists of \textit{rc} sentences and \textit{pp} sentences. We still obtain \textit{pp} sentences by copying from original QA-COGS and generate \textit{rc} sentences by adding a random relative clause into 2000 sampled QA-COGS sentences. The \textit{rc} is generated by using a random passive verb(e.g.\textit{ that was painted}). The generalization set for \textit{rc\_pp} is then generated by a heuristic similar to \textit{cc\_cp}. Our generated sentences share the same vocabulary with original COGS sentences and we control all clauses depth always being 1, so there is no length generalization in our datasets. 
% The train set of \textit{cc\_cp} consists of two parts. The first part is copied exactly from the original train set of QA-COGS. The second part 

% Noticing that current questions are not enough to test the structural generalization for compositionality, we extend the corpus with two new structural generalization types, named as \textit{cc\_cp} and \textit{rc\_pp}. Specifically, we introduce relative clause and coordination structures into the train set of QA-COGS and test their combination with prepositional phrase and complement clause respectively. 
% In addition to the questions we described in section \ref{sec:overview}, we also introduce coordination structure into our train set and combine the coordination structure with complement clause in the generalization set. 
\input{tables/coordination_cp_example} 

% An example of our idea can be seen in Table \ref{tab:coordination_cp_example}. For \textit{cc\_cp} type, a compositionality-aware model should be able to learn that the predicate \textit{jog} in the generalization example should be coordinated with \textit{like} according to the tense, and thus the answer will be \textit{that Noah discovers a boy}. However, a model that does not learn structural generalization will possibly answer \textit{that Noah discovers a boy and jogged}. Similarly, in \textit{rc\_pp}, the form of \textit{be} verb (i.e. \textit{was/were}) determines which noun is attached by the prepositional phrase, but a heuristic-based model cannot learn this. 

% To create test data for \textit{cc\_cp}, for a sentence containing complement clause in the original train set, we randomly sample an unergative verb and combine them with a coordination structure. An example can be seen in the first case of Figure \ref{fig:struct_example}. Note that to obtain an unambiguous sentence, we need to guarantee the main verb has a different tense from the clause verb(i.e. \textit{Oliver liked that Noah discovered a boy and jogged} is ambiguous). Thus, depending on the combination of tenses of main verb and clause verb, we generate 4 sentences for each original COGS sentence as our new test set. To create the train set, we randomly sample 2000 sentences without complement clauses from the original train set and add coordination structure to the sampled sentences. We then concatenate resulted sentences with original train set as new train set.  

% To create test data for \textit{rc\_pp}, for a sentence containing preposition phrase in the original train set, we randomly sample a verb that takes a noun as the argument and combine them with a relative clause. An example can be seen in the second case of Figure \ref{fig:struct_example}. Similar to the \textit{cc\_cp} case, we need to guarantee two nouns have different singular and plural forms and thus obtain 4 sentences for each original COGS sentence as our new test set. We also introduce relative clauses into 2000 sentences without prepositional phrase in the original train set and concatenate them as new train set. 

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/struct_example.png}
    \caption{Example of generating generalization data for \textit{rc\_cc} and \textit{cc\_cp}.}
    \label{fig:struct_example}
\end{figure}

% \todo{introduce how to create the dataset}

\subsection{Experiment Setup}

In addition to the models introduced in section \ref{subsec:seq2seq:setup}, we also train a syntax-aware BART-QA model named \textit{BART-QA+syn} to make comparison. Instead of selecting an arbitrary span from the context string, this syntax-aware model is given the gold constituent tree and then constrained to select a constituent span for both training and inference. 

\subsection{Results}

\input{tables/struct_gen_type_results}

The results are shown in Table \ref{tab:qa_struct_results}. We observe BART-QA now fails on these two new generalization dataset. We consider this is because different from the structural generalization types in section \ref{sec:overview}, our new datasets can not be solved by a string-level heuristic. For BART, our dataset is still difficult. Note that since we only have recursion depth being 1 in our new test data, this difficulty genuinely comes from the structural generalization rather than length generalization.  
% indicating the inability of seq2seq models to combine known structures. 
However, BART-QA+syn achieves great accuracy, which means that a syntax-aware model is robust in structural generalization. 

\input{tables/rc_example}

Looking into the output of BART and BART-QA, we find both models tend to output the same span with different \textit{be} verb forms as shown in Table \ref{tab:error_rc}. We consider this is because models without structure bias directly learn to select the span on the left of the relative clause. 

% We apply the same models as in section \ref{subsec:seq2seq:setup} on our new corpuses. 
% The results is shown in Table \ref{tab:qa_struct_results}. Note that our introduced structure (e.g. coordination structure) could be attached to the verb either in the main sentence or the clause. We report the accuracy for the two categories separately as \textbf{main} and \textbf{sub}. 

% \todo{Remember we have many possible splits for \textit{cc\_cp}.  Which setting and results should we present here? }

% \todo{I found that when we test BART model on \textit{cc\_cp} type, the model always outputs the complement clause without the coordination structure. Maybe it is because our training samples do not contain \textbf{\textit{and}} in the output side. I now plan to change the questions for cc\_cp type to avoid this problem. I will finish this section after that. }

% \paragraph{results} To be updated.
% \todo{Introduce the extractive model }

% \paragraph{\textcolor{red}{Connection with extractive model}} We have spent much efforts on exploring performance of extractive models on QA-COGS. However, I am now very confused on how to connect that work with the current story. I developed the extractive model because our initial story is to present a QA corpus, and thus we need to experiment with seq2seq, extractive and structured models. If our story now is \textit{seq2seq is not good at compgen}, then why do we need to present results of extractive models in this story?


==> EMNLP 2022/sections/QA_results.tex <==
%\pagebreak

\section{Experiments on \cogsqa} \label{sec:qa_experiments}


\subsection{Models} \label{subsec:seq2seq:setup}

We conduct a series of experiments in which a model receives the concatenation of context sentence and question as input and must predict the answer. 
We fine-tune BART and T5 on \cogsqa\ and compare against two \linf\ models. Details of the training setup are discussed in Appendix \ref{appendix:sec:train}.

First, we compare against an extractive model we call BART-QA. Given a context sentence and question, BART-QA predicts the start and end position of the answer within the context sentence. The start and end positions are each predicted by an MLP trained from scratch which takes the outputs of the pretrained BART encoder as input.

% one consecutive span from the context sentence as the predicted answer. BART-QA consists of the pretrained BART encoder and two multi-layer perceptrons (MLP) trained from scratch. During training, token representations from the encoder are fed into the two MLPs to predict a score for being the start and end index of the span independently. During inference, we simply select the most possible start and end index independently.

Second, we use a more informed model called BART-QA+struct specifically for \cogsqacc. {BART-QA+struct} shares the same encoder as {BART-QA}, but its decoder is constrained to select a span which exists in the gold syntax tree of the sentence. This model accesses information that is usually not available at test time, and we offer it only as a point of comparison.


% . Instead of selecting an arbitrary span from the context string, the decoder here is given the gold constituent tree and constrained to select a constituent span for both training and inference. We admit this is not a realistic setting, and only use this experiment to show benefits from a task-specific decoder with enough linguistic knowledge.  

% To solve \textit{cc\_cp} dataset, the model need to learn to combine structures. However, both seq2seq and BART-QA are not designed to be explicitly aware of structures. Thus we further train a structure-aware model named \textit{BART-QA+syn} on \textit{cc\_cp} to see if it can solve \textit{cc\_cp}. \textit{BART-QA+syn} shares the same encoder as \textit{BART-QA}, but uses a structured decoder. Instead of selecting an arbitrary span from the context string, the decoder here is given the gold constituent tree and constrained to select a constituent span for both training and inference. 

\subsection{Results}


The exact match accuracies on the generalization sets are shown in Table \ref{tab:qa_gentype_eval}. Similar to the earlier experiments, all models perform well on \lexg; we mainly discuss results on \structg below. 

\paragraph{\cogsqabase.} All models solve ``Object to Subject PP'' perfectly, with T5 and BART-QA also achieving perfect accuracy on the PP and CP recursion. While these positive results on structural generalization seem to go against the grain of our earlier discussion, it is important to note that \cogsqabase\ is an extractive task which only requires selecting a substring of the input; and further, that this substring is in a very specific position of the string, making the task amenable to learning simple heuristics (e.g.\ subject is everything to the left of the verb). Thus, these results indicate that structural generalization is hard only if the decoder's task is sufficiently complex. Note that unlike BART, T5 sees question answering tasks during training, which may help explain the difference in accuracy.

\paragraph{\cogsqacc.} However, BART and T5 all achieve low accuracy on \cogsqacc, suggesting that even text-to-text tasks involving structural generalization can be difficult; string-level heuristics are not successful on this task. In this case, the task is still hard for the \linf\ model BART-QA. It can be solved by BART-QA+struct, but note that this model has access to gold syntax information which makes the task much easier.
Note that since the training and generalization sentences in \cogsqacc\ are of similar length, the difficulty comes exclusively from structural rather than length generalization.






% we only have recursion depth being 1 in our new test data, this difficulty genuinely comes from the structural generalization rather than length generalization.  




% \paragraph{Obj to Subj PP} Different from the pattern in parsing and tagging tasks, both seq2seq and BART-QA models solve the Obj to Subj PP type. To see why this difference happens, we present an example for this generalization type in Table \ref{tab:qa_gen_examples}. We notice that our task does not require the model to be aware of syntactic structure to answer the question(i.e. the agent of a predicate is usually the string on the left of itself). Thus, even though PP modified noun phrases never appear during training, the model can learn this "shallow" heuristic to answer most questions correctly. 

% \paragraph{Recursion generalization is still difficult} We also observe that CP and PP recursion generalization types are still difficult for BART but not for T5. We consider the high accuracy of T5 is because it is trained on supervised question answering tasks during pretraining. We thus mainly focus on the result of BART. Although the example in Table \ref{tab:qa_gen_examples} almost requires no structural knowledge(i.e. the model only needs to generate the context string on the right of \textit{said}), BART still struggles to solve it. This suggests that seq2seq models cannot do length generalization correctly, even in our simple generation task. On the other hand, BART-QA performs well on such types, which is consistent with the pattern of \linf\ models. 

% To better show the behaviour of seq2seq in such generalization types, we further present the BART result on CP recursion type with regard to different recursion depth in answer and context in Figure \ref{fig:qa_ans_depth}. Note that our train data only contains answers with depth up to 1, and the generalization data contains data with gold answer depth being up to 12. The figure shows that the accuracy decreases as the answer depth grows for all context depths, which means that the model struggles to generate longer sequence. However, for a fixed answer depth, we do not find a clear pattern on accuracy with regard to different context depth. 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.42]{figures/qa_recursion_answer_depth.pdf}
%     \caption{Exact match accuracy of BART on CP recursion typed questions. Answer depth  denotes the number of CP recursions in the answer. \textit{sent depth} denotes the recursion number in the context.}
%     \label{fig:qa_ans_depth}
% \end{figure}

% % \input{tables/struct_gen_type_results}

% \paragraph{Distinguish structure combinations}
% We then report the sequence-level accuracy (average over four splits) on \textit{cc\_cp} and \textit{rc\_pp} in corresponding columns in Table \ref{tab:qa_gentype_eval}. We observe BART-QA fails on these two datasets. We consider this is because different from the structural generalization types in original COGS, our new datasets can not be solved by a string-level heuristic. For BART, our dataset is still difficult. Note that since we only have recursion depth being 1 in our new test data, this difficulty genuinely comes from the structural generalization rather than length generalization.  
% BART-QA+struct achieves great accuracy, which means that a \linf\ model is robust in structural generalization. 

% \input{tables/rc_example}

% Looking into the output of BART and BART-QA, we find both models tend to output the same span with different \textit{be} verb forms as shown in Table \ref{tab:error_rc}. We consider this is because models without structure bias directly learn to select the span on the left of the relative clause. 

==> EMNLP 2022/sections/QA_study.tex <==

\section{Text-to-text structural generalization} \label{sec:overview}

We will now turn our attention to a novel text-to-text variant of COGS. The difficulty of structural generalization for seq2seq models has been primarily studied on tasks where sentences must be mapped into symbolic representations of some kind, such as the semantic and syntactic representations in Section~\ref{sec:semantic-parsing}. But although pretrained seq2seq models like BART and T5 achieve excellent accuracy on broad-coverage semantic parsing tasks, one might argue that they were originally designed for tasks where the output sequence is natural language as well, and thus should be evaluated on such tasks.

We therefore propose a new dataset, \cogsqa, which presents structural generalization examples based on COGS sentences in a question-answering format. Given a context sentence and a question sentence as input, the goal is to output the correct answer, which should be a consecutive span of tokens in the context sentence. The dataset consists of two sections: \emph{\cogsqabase} directly asks questions about COGS sentences (\cref{subsec:arg_rel}), whereas \emph{\cogsqacc} combines COGS sentences in novel coordinating structures (\cref{subsec:cc_cp}). Following the original COGS design, each section consists of four subsets: training set, development set, in-distribution test set, and out-of-distribution generalization set. 


\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/cc_cp_example.pdf}
    \caption{Construction of \cogsqacc: top is \textit{cc\_cp}, bottom is \textit{rc\_pp}. The answer to the example question is highlighted in bold.
% \todo{fix picture}  
 }
    \label{fig:cc_cp_example}
\end{figure}

\input{tables/qa_gen_examples}

\subsection{\cogsqabase} \label{subsec:arg_rel}
The \cogsqabase\ dataset uses the sentences of COGS as context sentences, and then asks one or more questions about each sentence that can be answered by a contiguous substring (see Fig.\ \ref{fig:qa_gen_examples}). For example, given \textit{Noah ate the cake on the plate} as context, we ask \textit{What did Noah eat?} and \textit{Who ate the cake on the plate?}, and the answer should be \textit{the cake on the plate} and \textit{Noah} respectively.

To generate question-answer pairs, we identify the semantic roles and arguments for each predicate in all sentences of COGS, as in the SRL probing task (\cref{sec:probing-howto}). We generate question-answer pairs out of these based on handwritten templates (i.e.\ at least one per COGS instance) and split them into train/test/generalization sets as in the original COGS. We refer to Appendix \ref{appendix:sec:qa} for more details.

The original COGS training set contains ``primitive'' instances in which the sentence consists of a single word, and the meaning representation is the word itself (e.g.\ Paula $\Rightarrow$ Paula). We include these instances in \cogsqabase\ by using a special token \textit{<prim>} as the question sentence and the primitive word as context and answer (i.e., Paula \textit{<prim>} $\Rightarrow$ Paula).


%\todo{add dataset statistics in appendix}

% \paragraph{Argument Relation} \label{para:arg_relation} For each sentence, we generate a question to ask the argument relations in a predicate. To generate the corpus, we first label each verb predicate in COGS sentences with their frames from the gold meaning representations, and then map each predicate-argument pair into a question-answer pair based on predefined templates. Note that the preposition phrase in COGS can only modify the noun phrases, and thus there is no \textit{location} argument for verb predicates . We do this generation process for all sets (i.e. train/dev/test/gen), which results in 54206 train sentences, 6834 dev sentences, 6798 test sentences and 67989 generalization sentences. 


\input{tables/QA_results}


\subsection{\cogsqacc} \label{subsec:cc_cp}
We add \cogsqacc\ as a second, harder text-to-text task based on COGS. This task exploits the interplay of the syntactic structure of a sentence with constraints on tense and number agreement. For instance, in sentences of the form ``N1 V1 that N2 V2 and V3'' (where N1, N2 are noun phrases and V1, V2, V3 are verbs),
V3 belongs to the same clause as V1 or V2 depending on which one it agrees with. Thus, the agreement between verbs disambiguates a structural ambiguity of the sentence. Some concrete examples are shown in Fig.~\ref{fig:cc_cp_example}. The idea that agreement interacts with syntax is reminiscent of \citet{linzen2016assessing}, but here we predict the syntactic structure rather than the agreement feature.

\cogsqacc\ consists of two parts. The subcorpus \textit{cc\_cp} consists of sentences as above, where tense agreement disambiguates the structural ambiguity between CP embedding and coordination. The subcorpus \textit{rc\_pp} contains sentences where number agreement disambiguates the attachment of a relative clause. In both cases, we construct context sentences using a context-free grammar adapted from the one that generates COGS. We generate questions of the form ``What is the ccomp of said?'' along with their answers from the context sentences using a small number of hand-written heuristics.  Answering these questions correctly amounts to disambiguating the structure of the sentence.

We create training (4k instances), development (1k), and in-domain test sets  (1k) for \cogsqacc\ out of three of the four combinations of the agreement features of the two verbs (white cells in Fig.~\ref{fig:cc_cp_example}). We create a generalization set (2k instances) from the fourth, unseen combination of agreement features (gray cells).
% \todo{Does everyone get perfect accuracy on the in-domain test set?}







% We introduce the dataset \textit{cc\_cp} here to explore generalization to combination of coordination structure and complement clause. Different from context sentences in the dataset described in section \ref{subsec:arg_rel}, here we introduce coordination structure and present tense into the grammar of context sentences.  An overview of this dataset is shown in the left table in Figure \ref{fig:cc_cp_example}. For the question-answer pairs, we only use question \textit{What is the ccomp of V\_cp}, where \textit{V\_cp} denotes the verb taking the complement clause. In practice, this dataset has four different splits, each of which has one cell in Figure\ref{fig:cc_cp_example} being the generalization set and the rest three being the in-distribution sets.  
 
% The idea of this dataset is different from the structural generalization types in Figure \ref{fig:qa_gen_examples}, where the context sentences contain novel combination of seen structures(i.e. pp recursion). In the generalization set of \textit{cc\_cp}, two familiar structure combinations exist in one context sentence, both of which are seen during training. The model need to learn to distinguish these two combinations depending on the verb tenses in the sentence. For example, for the bottom-right sentence in Figure \ref{fig:cc_cp_example}, the answer for question \textit{What is the ccomp of Oliver ?} should be \textit{that Noah discovered a boy and slept}, since verb tenses inside the coordination structures should be the same. We consider this dataset as structural generalization too.

% Similar to \textit{cc\_cp}, we introduce the relative clause (rc) structure and the plural forms of verbs in \textit{rc\_pp} dataset as shown in the right table in Figure \ref{fig:cc_cp_example}. This dataset also has four different splits and we only ask question \textit{What is the theme of V\_passive}, where \textit{V\_passive} denotes the passive verb in the relative clause. 

% % \subsection{Data creation} 
% % \paragraph{Argument relation} We use the COGS sentences as our context sentences for this dataset. To generate question-answer pairs, we first label each verb predicate in COGS sentences with their frames from the gold meaning representations, and then map each predicate-argument pair into a question-answer pair based on predefined templates. Note that the preposition phrase in COGS can only modify the noun phrases, and thus there is no \textit{location} argument for verb predicates.

% % % \paragraph{Primitives} 
% % The original COGS train set contains some primitives data where the input is a primitive word and the output is itself(i.e. Paula => Paula). To make such data fit our task, we use a special token \textit{<prim>} as the question sentence and the primitive word as context and answer(i.e. Paula \textit{<prim>} => Paula). Thus in our text generation tasks the model is still aware of primitive words.

% % \paragraph{\textit{cc\_cp} and \textit{rc\_pp}} 
% We use probabilistic context-free grammar to generate context sentences in this dataset. Question-answer pairs are extracted from the generated context sentences with hand-written heuristics. We control the recursion depth being 1 in both train and generalization sets for these two datasets.

% % \subsection{Setup}\label{subsec:seq2seq:setup}

% % \input{tables/QA_results}

% % We train BART as our model on QA-COGS.  To apply BART for the question answering task, we directly fine-tune the pretrained \textit{bart-base} model on it with the corresponding tokenizer. During fine-tuning, the model takes as input the concatenation of context and question strings and outputs the answer.

% % To see the how a non-seq2seq model behaves on QA-COGS, we also have another extractive model named BART-QA for comparison. Given a context and question sentence, BART-QA selects one consecutive span from the context sentence as the predicted answer. BART-QA consists of the pretrained BART encoder and two multi-layer perceptrons (MLP) trained from scratch. During training, token representations from the encoder are fed into the two MLPs to predict a score for being the start and end index of the span independently. During inference, we simply select the most possible start and end index independently.


% % \subsection{results}

% % We report sentence-level accuracy of QA-COGS in Table \ref{tab:selected_gentype_eval}. Similar to the case in parsing and tagging tasks, all models perform well on lexical generalization types. We thus focus on discussing results on structural generalization types below. 






% % We can observe that seq2seq models solve the predicate classification task, but still struggle on argument identification and relation tasks. We thus focus on discussing these results on these two tasks.

% % \input{tables/qa_detailed_results}

% % \paragraph{Lexical Generalization} We first look at argument relation task. Clearly, seq2seq solves most lexical generalization types except for \textit{prim\_to\_subj\_proper}, \textit{prim\_to\_obj\_proper} and \textit{prim\_to\_inf\_arg}. Looking into the output of the model, we find that errors for such primitive generalization types all come from the inability to copy the primitive as seen below. 
% % \begin{center}
% % \noindent\fbox{
% %     \parbox{.9\linewidth}{
% %     \textbf{Context} \textit{Noah imagined that Emma supported that Paula wanted to dance .}
    
% %     \textbf{Question} \textit{Who did Noah imagine that Emma support that want to dance ?}
    
% %     \textbf{Gold} \textit{Paula}
    
% %     \textbf{Pred} \textit{Paula Paula}
    
% %     }
% % }
% % \end{center}

% % Note that a primitive in original COGS is only annotated as either its word form or a lambda expression, so we cannot generate question-answer pairs for primitives in the train set. This means that such primitives (e.g. \textit{Paula} and \textit{crawl}) are out-of-vocabulary tokens for our model. We consider such errors are mainly due to the instability of fine-tuning our pretrained seq2seq models.
% % \todo{Do we need to use seq2seq with copy mechanism to get a better picture here?}
% % However, another question exists: why the model can meanwhile solve the common noun cases (e.g. \textit{prim\_to\_obj\_common})? Does BART have some internal weakness for proper nouns? We currently do not have a clear answer for this. \todo{ T5 does not have this issue so maybe this paragraph does not make much sense and we can just say it's the internal weakness of BART. Of course we can replace \textit{Paula} in the generalization set with other proper nouns to confirm this assumption.} T5 and extractive model perform well on this type. 

% % Now look at the argument relation task. Both extractive and seq2seq models cannot fully solve \textit{prim\_to\_obj\_proper}. However, we notice that for the same sentence, the two models make different types of errors as seen in the example below. \todo{Maybe I should add primitive word into the train set or try T5 on this task. This discussion does not make much sense to myself.} If extractive model cannot recognize Paula as a theme, how could it solve the argument relation task? Noticing that in relation task the question will become \textit{What did Emma sell the girl?}, we consider the extractive model simply learns to select the span not occurring in the question string. 

% % \begin{center}
% % \noindent\fbox{
% %     \parbox{.9\linewidth}{
% %     \textbf{Context} \textit{Emma sold the girl Paula .}
    
% %     \textbf{Question} \textit{What is the theme of sell ?}
    
% %     \textbf{Gold} \textit{Paula}
    
% %     \textbf{BART Pred} \textit{the girl}
    
% %     \textbf{BART-QA Pred} \textit{the girl Paula}
    
% %     }
% % }
% % \end{center}

% % \paragraph{Obj to Subj PP} Different from the pattern in parsing and tagging tasks, both seq2seq and BART-QA models solve the Obj to Subj PP type. To see why this difference happens, we present an example for this generalization type in Table \ref{tab:qa_gen_examples}. We notice that our task does not require the model to be aware of syntactic structure to answer the question(i.e. the agent of a predicate is usually the string on the left of itself). Thus, even though PP modified noun phrases never appear during training, the model can learn this "shallow" heuristic to answer most questions correctly. 

% % \paragraph{Recursion generalization is still difficult} We also observe that CP and PP recursion generalization types are still difficult for seq2seq models. Although the example in Table \ref{tab:qa_gen_examples} almost requires no structural knowledge(i.e. the model only needs to generate the context string on the right of \textit{said}), seq2seq models still struggle to solve it. This suggests that seq2seq models cannot do length generalization correctly, even in our simple generation task. On the other hand, BART-QA performs well on such types, which is consistent with the pattern of non-seq2seq models in NLU tasks. 

% % To better show the behaviour of seq2seq in such generalization types, we further present the result of CP recursion with regard to different recursion depth in answer and context in Figure \ref{fig:qa_ans_depth}. Note that our train data only contains answers with depth up to 1, and the generalization data contains data with gold answer depth being up to 12. The figure shows that the accuracy decreases as the answer depth grows for all context depths, which means that the model struggles to generate longer sequence. However, for a fixed answer depth, we do not find a clear pattern on accuracy with regard to different context depth. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[scale=0.3]{figures/qa_recursion_answer_depth.pdf}
% %     \caption{Exact match accuracy of BART on CP recursion typed questions. Answer depth  denotes the number of CP recursions in the answer. \textit{sent depth} denotes the recursion number in the context.}
% %     \label{fig:qa_ans_depth}
% % \end{figure}



==> EMNLP 2022/sections/Related_works.tex <==
\section{Related work}\label{sec:related_work}
%\paragraph{Compositional generalization in COGS.}

% Recently the limitations of seq2seq models in compositional generalization have gained great attention: \cite{lake-baroni-2018-generalization} show that seq2seq models cannot generalize to either novel combinations of seen words or length generalization on SCAN; \cite{hupkes2020compositionality} confirm this on an artificial translation task named PCFG; \cite{keysers-etal-2020-measuring} propose CFQ corpus based on compound divergence and find seq2seq also struggles on this corpus. 

The recent interest in compositional generalization has raised concerns about limitations of seq2seq models. For instance, the SCAN dataset \citep{lake-baroni-2018-generalization} requires a model to translate natural-language instructions into symbolic action sequences; it has multiple splits in which the test data contains new combinations of commands or instructions that are systematically longer than in training. The PCFG dataset \citep{hupkes2020compositionality} builds upon SCAN and adds instructions with recursive structure. The CFQ dataset \citep{keysers-etal-2020-measuring} maps questions to SPARQL queries, and splits the data according to a measure of compositional complexity (MCD). In all of these papers, simple seq2seq models based on LSTMs and transformers were shown to perform poorly when the test data was more complex than the training data.

Since then, followup research has shown that both generic transformer-based models \citep{ontanon-etal-2022-making,csordas-etal-2021-devil}, general-purpose pretrained models \citep{furrer-etal-2020-compositional}, and seq2seq models that are specialized for the task can achieve higher accuracies than the ones reported in the papers introducing the datasets. Nonetheless, there is a sense that despite the best efforts of the community, pure seq2seq models are hitting a ceiling on compositional generalization tasks. 

In this paper, we shed some light on the issue by (a) clarifying that seq2seq models do not struggle with compositional generalization per se, but with \emph{structural} generalization, and (b) demonstrating that this type of generalization remains hard for seq2seq models even after heavy pretraining. This is in contrast to most previous research, which has avoided pretraining and focused on length or MCD as the primary source of difficulty. Our data includes instances where the structure, but not the length differs between training and testing, and therefore allows us to differentiate between the two. The importance of structure to compositional generalization is also recognized by \citet{bogin-2022-local-structure}.
%; we show that it is not only an issue in semantic parsing, but in other tasks as well.

The difficulty of structural generalization for neural models has also been studied in more targeted ways. For instance, \citet{yu-etal-2019-learning} show empirically that LSTM-based seq2seq models cannot learn to close the brackets of Dyck languages, and \citet{hahn-2020-theoretical} proves that transformers cannot learn to distinguish well-bracketed Dyck expressions. 
\citet{DBLP:journals/tacl/McCoyFL20} find empirically that seq2seq models struggle to learn the structural operations necessary to rewrite declarative English sentences into questions, whereas tree-based models work better.

% A broader study also investigate the ability to generalize to hierarchical structures 

% Recent study on compositional generalization has gained great attention. Although many datasets and studies have been proposed such as SCAN\cite{lake-baroni-2018-generalization}, PCFG\cite{hupkes2020compositionality} and CFQ \cite{keysers-etal-2020-measuring}, only COGS\cite{kim-linzen-2020-cogs} considers structural generalization with syntactic structures in human languages. 

% \citet{kim-linzen-2020-cogs} demonstrate that simple
% seq2seq models (LSTMs and Transformers) struggle with all
% generalization types in COGS. Subsequent work with novel seq2seq
% architectures achieve a much higher mean accuracy on lexical generalization 
% types \citep{akyurek-andreas-2021-lexicon,csordas-etal-2021-devil,
%   conklin-etal-2021-meta,tay-etal-2021-pretrained,orhan-2021-compgen,
%   zheng-lapata-2021-disentangled}, but their accuracy on structural 
%   generalization types are still very low. On the other hand, \citet{liu-etal-2021-learning} and \citet{weissenhorn22starsem} show that such structural generalization can be solved by a model with a task-specific architecture. 

% Structural generalization has also been probed in syntactic tasks.
% %\pw{do we want to cite that superrecent \citet{goodwin-etal-2021-compositional} paper?} 
% \citet{linzen2016assessing} define
% a number-prediction task that requires learning syntactic
% structure and find that LSTMs perform with some success;
% however, \citet{kuncoro-etal-2018-lstms} find that structure-aware
% RNNGs perform this task more accurately.
% \citet{DBLP:journals/tacl/McCoyFL20} found that hierarchical representations are necessary for human-like syntactic generalizations on a question formation
% task, which seq2seq models cannot learn.





% Recently the limitations of seq2seq models in compositional generalization have gained great attention. \citet{lake-baroni-2018-generalization} creates a semantic parsing dataset SCAN, where the input is navigation commands(e.g.\ jump twice) and the output is an action sequence(e.g.\ JUMP JUMP). Their data is design to make the model generalize to novel compositions of commands which are not encountered during training. For example, the train set contains a primitive command (e.g.\ jump) and other commands(e.g.\ run, run twice), and the test set contains commands composed of the primitive command(e.g.\ jump twice). They also provides a length split which requires generating longer sequence than those seen during training. Their study shows simple recurrent network (SRN)\cite{elman1990finding}, long short-term memory network (LSTM)\cite{hochreiter1997long} and gated recurrent units (GRU)\cite{69e088c8129341ac89810907fe6b1bfe} based seq2seq models struggle on the dataset. \citet{hupkes2020compositionality} confirms this by proposing a new dataset PCFG and experimenting LSTM, Transformer \cite{vaswani2017attention} and convolution based seq2seq models. \citet{keysers-etal-2020-measuring} also proposes a dataset CFQ, where the data split is designed to maximize the difference of compositions between train and test set. Their study also suggests that LSTM and Transformer based seq2seq have limitations on compositional generalization. Compared to these studies, our work focuses on human-like structural generalization in natural language grammars and we use powerful pretrained seq2seq models. Although \citet{hupkes2020compositionality} also studies generalization to deeper structures, the length of their sentence grows with larger depth. By contrast, the Obj\_to\_Subj\_PP in our dataset allows us to explore structural generalization without length generalization. 

% Despite these studies, some follow-up works show that the generalization ability of seq2seq models have been underestimated on these datasets. \citet{furrer-etal-2020-compositional} apply T5 models across different datasets and find pretraining helps compositional generalization to some extents; \citet{ontanon-etal-2021-making} and \citet{csordas-etal-2021-devil} explore the design space of Transformers and find relative position encoding useful \cite{shaw-etal-2018-self}. Our study is also based on pretrained transformers(i.e. BART and T5). However, our study suggests that neither pretraining nor better designed transformers\cite{csordas-etal-2021-devil} improve structural generalization.


% % I think we don't need this - AK
% % Different from these studies, our work focuses on human-like structural generalization in natural language grammars. Recent works have proposed many methods to improve the performance on datasets above\citep{akyurek-andreas-2021-lexicon,csordas-etal-2021-devil,  conklin-etal-2021-meta,tay-etal-2021-pretrained,orhan-2021-compgen,  zheng-lapata-2021-disentangled}, but we show that none of them helps in structural generalization. Note that structural generalization is different from length generalization. Although recursion generalization types require longer output sequence, Obj to Subj PP generalization output has the same output length as training data and its difficulty completely comes from the novel combination of structures.  

==> EMNLP 2022/sections/Semantic_Parsing.tex <==
\section{Structural generalization is hard for seq2seq}
\label{sec:semantic-parsing}

We begin with some evidence that structural generalization in COGS is hard for seq2seq models, while \linf\ models learn it quite easily. We first collect some results on the original semantic parsing task of COGS, extending it with numbers for BART and T5. We then transform COGS into a corpus for syntactic parsing and POS tagging and investigate the ability of BART and T5 to generalize structurally on these tasks.


\subsection{Experimental setup: COGS}\label{subsec:first:setup}

We follow standard COGS practice and evaluate all models on the generalization set.
We report exact match accuracies, averaged across 5 training runs.

\paragraph{Seq2seq models.} \label{subsec:seq2seq:setup}
We train BART \cite{lewis-etal-2020-bart-acl} and T5 \cite{raffel-etal-2020-t5} as semantic parsers on COGS. Both models are strong representatives of seq2seq models and perform well across many NLP tasks.
To apply these models on COGS, we directly fine-tune the pretrained
\textit{bart-base} and \textit{t5-base} model on it with the corresponding tokenizer; see Appendix \ref{appendix:sec:train} for details.
We also report results for a wide range of published seq2seq models for COGS
\citep{kim-linzen-2020-cogs,conklin-etal-2021-meta,csordas-etal-2021-devil,akyurek-andreas-2021-lexicon, zheng-lapata-2022-disentangled, qiu2021improving}.

\paragraph{\Linf\ models.}  We report evaluation results for LeAR \citep{liu-etal-2021-learning} and the AM parser \citep{weissenhorn22starsem}. Both models learn to predict a tree structure which is decoded into COGS meaning representations using the Principle of Compositionality. Thus both models are \linf.

\input{tables/COGS_results_official}


\subsection{Results}
We report the results by generalization type in the ``semantic'' rows in  \Cref{tab:selected_gentype_eval}. We will explain ``BART+syn'' in
\cref{subsec:seq2seq:semantic_gen_with_syntax} and the ``syntactic'' and ``POS''
sections in \cref{subsec:seq2seq:syntactic_gen}.

\paragraph{Structural generalization is hard.} We can observe that all recent models achieve near-perfect accuracy on the 18 lexical generalization types. However, all pure seq2seq models achieve very low accuracy on the structural generalization types, whereas \linf\ models are still very accurate.
One outlier is the seq2seq model of \citet{qiu2021improving}. It employs heavy data augmentation based on (\linf) synchronous grammars encoding the Principle of Compositionality, which provides training instances of higher recursive depth to the seq2seq model. The seq2seq model then still generalizes to the recursive depth which it has seen in training, but not beyond (Peter Shaw, p.c.).

Note that the mean accuracy is dominated by the lexical generalization types; to really measure the ability of a model to generalize to unseen structures, it is important to focus on the structural generalization types. Note further that BART and T5 perform very well among the class of seq2seq models, outperforming many models that are specialized to COGS. We will focus on these two models in the experiments below.

It is important that although the generalization instances on PP and CP recursion are longer than the training instances, the low accuracy of the seq2seq models cannot be explained exclusively in terms of their known weakness to length generalization \citep{hupkes2020compositionality}. For the ``Object to Subject PP'' generalization type, the generalization and training sentences have the same length, but different structures. Thus our results point towards a specific weakness to structural generalization.

% \paragraph{Structured models outperform seq2seq.}
% We observe that all
% structured models outperform all seq2seq models on the
% generalization set by a wide margin, including strong pretrained BART and T5 models. LeAR even achieves its near-perfect accuracy when trained on `train',
% and outperforms all seq2seq models trained on either dataset. 


% \paragraph{Performance by generalization type.}
% To understand this result more clearly, we break down the accuracy by
% generalization type. This analysis is shown in
% \cref{tab:selected_gentype_eval}.  We will explain ``BART+syn'' in
% \cref{subsec:seq2seq:semantic_gen_with_syntax} and the ``syntax''
% rows in \cref{sec:syntax}. We compare the
% compositional models against all seq2seq models that report these
% fine-grained numbers or for which they were easy to reproduce\todo{add Appendix}.


% The results group neatly with the three classes of generalization types
% outlined in \cref{sec:background}: \textsc{Lex}, \textsc{Struct}, and \textsc{Prop}. All recent models achieve
% near-perfect accuracy on each of the 16 lexical generalization
% types. On structural generalization types, seq2seq models achieve very
% low accuracies, whereas the structured parsers
% are still very accurate. The proper-noun object cases are somewhere in
% the middle, with the seq2seq models reporting middling numbers.
% % We revisit this class in \cref{sec:analysis-extensions}.


\paragraph{Depth generalization.}
The accuracy of the seq2seq models depends on the difference in complexity of the test instance and the training data. For instance, all training instances for the ``PP recursion'' type have recursion depth two or less; \cref{fig:depths_plot} shows how the accuracy depends on the recursion depth of the test instance. As we see,
the accuracy of BART (even when informed by syntax, cf.\
\cref{subsec:seq2seq:semantic_gen_with_syntax}) degrades
quickly with recursion depth. By contrast, LeAR and the AM parser
maintain high accuracy across all recursion depths.



% . This
% suggests that they learn the correct structural generalizations even
% from training observations of limited depth.

\begin{figure}
    \centering
    % you can surround the include command with \fbox{...} to get a border around the space used by the image
    % trim{left lower right upper}, clip   together crops the image
    \includegraphics[scale=.3,trim={5mm 5mm 40mm 0},clip]{figures/recursion_depth.pdf}
    \caption{Influence of PP recursion depth on overall PP depth
      generalization accuracy. 
    %   \todo{This figure need to be changed to fit the current paper.}
    }\label{fig:depths_plot}
  \end{figure}
  


\subsection{\syncogs\ and \poscogs} \label{sec:syntax}
\label{subsec:seq2seq:syntactic_gen}
While these results on semantic parsing are suggestive, they could be explained away in many ways. For instance, the weakness of seq2seq models with respect to structural generalization might be specific to semantics, or the semantic representations chosen in COGS might be idiosyncractic and unfair to seq2seq models.

We therefore investigate structural generalization on a syntax variant of COGS. We convert each training and generalization instance of the COGS corpus into a pair of the sentence with its syntax tree (\syncogs) and a pair of the sentence with its POS tag sequence (\poscogs). This is possible because COGS is generated from an unambiguous context-free grammar; we reconstruct the unique syntax trees that underly each instance in COGS.

We replace the very
fine-grained non-terminals (e.g.\  \lform{NP\_animate\_dobj\_noPP}) of
the original COGS grammar with more general ones (e.g.\ \lform{NP}) and remove
duplicate rules (e.g.\ \lform{NP}$\to$\lform{NP}) resulting from this. 
We extract the POS tag sequences from the preterminal nodes of the syntax trees.
% For POS tagging sequences, we directly extract them from the processed syntactic
% annotations.

We train BART and T5 to predict linearized constituency trees 
and the POS tag sequences from the
input sentences. As a \linf\ model, we use the 
Neural Berkeley
Parser \citep{kitaev-klein-2018-constituency}, which consists of a self-attention
encoder and a chart decoder and therefore has the notion of a tree and its recursive structure built into the parsing model. 
On the POS tagging task, our ``\linf'' model is constrained to predict exactly one POS tag for each input token. Specifically, we determine the most frequent POS tag in the training data for each word type and assign it to all occurrences of the word during inference.

% we map a token into one POS tag in a dictionary through train set(i.e. \{\textit{eat: V, Noah: N, ...}\}) and use this dictionary to predict the sequence one-by-one during inference. 

\paragraph{Results.}
The results are shown in the  ``syntactic'' and  ``POS'' rows of
\cref{tab:selected_gentype_eval}. We find the same pattern as in the
semantic parsing case: the seq2seq models do well on
\lexg, but struggle with \structg. The \linf\ models 
handle all generalization types well.
Thus, the
difficulties that seq2seq models have on structural generalization on
COGS are not limited to semantics: rather, they seem to be a general
limitation in the ability of seq2seq models to learn linguistic
structure from structurally simple examples and use it
productively. 

% \subsection{Error analysis}

\input{EMNLP 2022/tables/obj_to_subj_pp_error}

We also present an example for \textit{obj\_pp\_to\_subj\_pp} type across different tasks in Figure \ref{fig:error_example}. For a sentence \textit{The baby on a tray in the house screamed}, T5 consistently predicted wrong symbol sequences. For example, in semantic parsing, T5 tends to predict \textit{tray} as the theme of \textit{scream} with a PP structure. This might be due to a preference of T5 to reuse the pattern for object-PP sentences in the train set even if the intransitive verb does not license it. T5 also displays an unawareness
of word order that is reminiscent of the difficulties that seq2seq models otherwise face in relating syntax to word order \citep{DBLP:journals/tacl/McCoyFL20}. For recursion generalization types, we find that the main error is that the decoder cannot generate long or deep enough sequences. 

% We consider this is because the novel structure in source language results in some unseen orders of symbols, which cannot be easily generalized with a sequential generation manner. For example, in the POS task, \textit{P} tag is always generated after \textit{V} during training, and the model might capture this irrelevant feature. For recursion generalization types, we find that the main reason is that the decoder cannot generate long or deep enough sequences.  

==> EMNLP 2022/sections/Syntax_pos_probing.tex <==

\section{Encoder or decoder?}
\label{sec:probing}

We now turn to the second question: \emph{Why} do seq2seq models struggle on structural generalization? We start by investigating at which point the model loses the structural information -- does the encoder not represent it, or can the decoder not make use of it? This also addresses an apparent tension between our findings and previous work demonstrating that pretrained models contain rich linguistic information \cite{hewitt-manning-2019-structural,DBLP:conf/iclr/TenneyXCWPMKDBD19}, which should be sufficient to at least solve \syncogs.



% , we explore whether the failure of seq2seq models is because the decoder does not learn to exploit such information, or because the encoder does not contain enough information for COGS. To do this, we probe the encoder of BART on COGS with two linguistic tasks. 
% However, previous works do show that such pretrained language models contain rich linguistic information that should be useful on COGS \cite{hewitt-manning-2019-structural, https://doi.org/10.48550/arxiv.1905.06316}. Does the failure of our seq2seq models come from the inability to exploit such linguistic information? Or is it because the COGS grammar is too strange and thus not learnt by the language model during pretraining? We investigate this question by probing the encoder of our pretrained seq2seq models on COGS. 

\subsection{Probing for structural information}
\label{sec:probing-howto}
We use the well-established probe task methodology \cite{peters-etal-2018-dissecting,tenney-etal-2019-bert} to analyze what information is present in the outputs of the BART encoder. We define both a syntactic and a semantic probing task:

\paragraph{Constituent labeling.} The goal of this task is to predict correct labels for all constituency spans in a sentence. We treat spans that are not constituents as if they were annotated with the \textit{None} label. The gold annotations are derived from \syncogs.


% same corpus in section \ref{sec:syntax} as gold annotations.
% We annotate illegal spans with \textit{None} label and thus make predictions for all possible spans. We use the same corpus in section \ref{sec:syntax} as gold annotations.

\paragraph{Semantic role labeling.} To measure the presence of structural semantic information, we define a probe task that predicts role labels for all predicate-argument relations in a sentence. For example, in the sentence \textit{Emma slept}, the goal is to recognize that \textit{slept} is a predicate with \textit{Emma} being its \textit{agent}. This task captures most of the information in the original COGS meaning representations as relations between tokens in the sentence. We extract data for this task (given two tokens, predict if the second is an argument of the first and with what role label) from the COGS meaning representation. We refer to  Appendix \ref{appendix:sec:srl} for details.
% We describe more details about our probe tasks in Appendix \ref{appendix:sec:train}.

We train probe classifiers in a similar way as \cite{tenney-etal-2019-bert}. For each task, we train a multi-layer perceptron to predict the target label from the outputs of the frozen pretrained encoder. For constituent labeling, 
the MLP reads a span representation obtained by subtracting the encodings of the tokens at the span boundary from each other \cite{stern-etal-2017-minimal}.  For semantic role labeling, the input of the MLP is the concatenation of the encodings for the predicate and argument token.

We evaluate the probes in two ways. First, we train the probes on the original training split of COGS  (``orig'').  However, this conflates the presence of structural information in the encodings with the ability of the probing MLP itself to perform structural generalization. We therefore also evaluate on a second split (``probe'') in which we add 60\% of the generalization set (randomly selected) to the training set and 10\% to the development set and keep the rest as the probe test set. This makes the probe test set in-distribution with respect to the probe training set. The encoder remains frozen and can therefore not adapt to the modified training set; we still obtain meaningful results about whether the pretrained encodings contain the information that is needed to learn to predict structure in COGS.


% In probing method, the performance on an in-distribution test set is used to evaluate how much linguistic information is encoded in the frozen encoder for the probe task. However, our goal here is to detect the information of the out-of-distribution set(i.e. generalization set).
% To address this issue, we randomly split the generalization set with 60\% being concatenated with the train set, 10\% being concatenated with the development set and the remaining as probe test set. To make comparison, we also experiment with original split while freezing the encoder. This means that the input for the decoder are the same in both \textit{probe} and \textit{orig} data settings.

\subsection{Results}
We report the sentence-level accuracy in Table \ref{tab:probe_eval}. 
For better comparison, all accuracies are measured on the test set from the ``probe'' split.
We find that the probes learn to solve both tasks accurately on the ``probe'' split, indicating that the pretrained encodings of BART contain all the information that is needed to make structural predictions. By contrast, when we replace the BART encodings with random vectors of the same size (``Random'' rows), the probe fails to learn. The probes also perform badly on the ``orig'' split, suggesting that the probe ``decoder'' does not generalize structurally either.

These findings suggest that the BART encoder captures all the necessary information about the input sentence, but the BART decoder cannot use it to learn to generalize structurally. 



% To show the high accuracy genuinely comes from encoded representations rather than the decoder, we experimented another encoder type \textit{Random}, where encoded representations are replaced with random initialized vectors with the same size. We can see that the model performs well in the probe setting for both span labeling and SRL tasks. This indicates that the pretrained encoder does contain enough linguistic information for COGS. However, when using the original train set, the performance on structural generalization types degrades quickly. This means that although the encoder already contains enough information to solve a task, the decoder may not learn to exploit these information with an unbalanced train set. 

% This suggests that although representations from the encoder are informative enough, the decoder(i.e. MLP classifier) cannot learn to exploit such information when given an unbalanced (i.e. compositional) data split. We thus conclude that decoder is the bottleneck of applying pretrained models in compositional generalization. 

\input{tables/probe_results}


% \subsection{Compositional generalization from correct
%   syntax}\label{subsec:seq2seq:semantic_gen_with_syntax}
\subsection{Enriching seq2seq with structure}\label{subsec:seq2seq:semantic_gen_with_syntax}

Can we make things easier for the decoder by making the structural information explicit in the input? To investigate this, we inject the gold syntax tree into the BART encoder to see if this improves structural generalization in semantic parsing.
%\todo{The MTL method may not fit this story quite well. }

% But perhaps the poor performance of seq2seq semantic parsers on
% \structg\ is caused \emph{only} by their inability to learn to
% generalize syntactically? Would their accuracy catch up with that of
% structured models if we gave them access to syntax?

We retrain BART on COGS, but
instead of feeding it the raw sentence, we provide as input the
linearized gold constituency tree (``\lform{(NP ({Det} a) ({N} rose))}''),
both for training and inference.
 This method is similar to 
\citet{li-etal-2017-modeling} and \citet{currey-heafield-2019-incorporating},
but we allow attention over special tokens such as ``\lform{(}'' during decoding.
% This method augments the feature representations in the encoder. 

We report the results as ``BART+syn'' in
\cref{tab:selected_gentype_eval} and \cref{fig:depths_plot}; the overall accuracy increases by
1.5\% over BART. This
is mostly because providing the syntax tree allows BART to generalize
correctly on \lexg. 
However, \structg remains out
of reach for BART+syn, confirming the deep difficulty of
structural generalization for seq2seq models.

We also explored other ways to inform BART with syntax, through
multi-task learning \cite{sennrich-etal-2016-controlling,
  currey-heafield-2019-incorporating} and syntax-based masking in the
self-attention encoder \cite{kim-etal-2021-improving}. Neither method
substantially improved the accuracy of BART on the COGS generalization
set (+1.0\% and -6.4\% overall accuracy, respectively). 
We conclude that the weakness of the BART decoder towards structural generalization persists even when the input makes the structure explicit.


==> EMNLP 2022/tables/COGS_results.tex <==
\begin{table*}
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
\begin{tabular}{@{}lll|ccc|cc|c|c@{}}
\toprule
& & Class & \multicolumn{3}{c|}{\structg} & \multicolumn{2}{c|}{\propg} & \lexg & \\
& & Gen. type & Obj to Subj PP & CP recursion & PP recursion & prim to
                                                               obj
                                                               (proper)
  & subj to obj (proper) & all 16 other types & Overall \\ 
\midrule
\parbox[t]{1mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{sem}}} 

& BART & train100 & \asbar{0} & \asbar{0} & \asbar{10} & \asbar{55} & \asbar{86} & \asbar{99} & \asbar{83} \\
& BART+syn & train100 & \asbar{0} & \asbar{7} & \asbar{8} & \asbar{98} & \asbar{95} & \asbar{100} & \asbar{86} \\ 
&T5 & train & \asbar{0} & \asbar{0} & \asbar{5} & \asbar{71} & \asbar{70} & \asbar{100} & \asbar{83} \\ 
&T5+aug & train & \asbar{0} & \asbar{64} & \asbar{46} & \asbar{89} & \asbar{89} & \asbar{100} & \asbar{90} \\ 
& LeAR & train & \asbar{93} & \asbar{100} & \asbar{99} & \asbar{93} & \asbar{93} & \asbar{100} & \asbar{99} \\ 
\cmidrule{2-10}
& \citealt{kim-linzen-2020-cogs} & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{30} & \asbar{45} & \asbar{35} \\
%& \citealt{ontanon-etal-2021-making} & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{51} & \asbar{43} & \asbar{56} & \asbar{48} \\ % table : rel2-eb-c small-6s seq2seq (not the strongest seq model, but strongest with per gen type results)
& \citealt{akyurek-andreas-2021-lexicon} & train & \asbar{0} & \asbar{0} & \asbar{1} & \asbar{66} & \asbar{64} & \asbar{100} & \asbar{82} \\
& \citealt{orhan-2021-compgen} & train & \asbar{0} & \asbar{0} & \asbar{10} & \asbar{84} & \asbar{86} & \asbar{100} & \asbar{85} \\
& \citealt{zheng-lapata-2021-disentangled} & train & \asbar{0} & \asbar{12} & \asbar{39} & \asbar{92} & \asbar{91} & \asbar{100} & \asbar{89} \\
& \citealt{kim-linzen-2020-cogs} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{23} & \asbar{54} & \asbar{77} & \asbar{63} \\
& \citealt{conklin-etal-2021-meta} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{20} & \asbar{66} & \asbar{94} & \asbar{75} \\
& \citealt{csordas-etal-2021-devil} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{55} & \asbar{62} & \asbar{92} & \asbar{75} \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{syn}}} & BART & train100 & \asbar{1} & \asbar{4} & \asbar{8} & \asbar{97} & \asbar{94} & \asbar{96} & \asbar{83} \\
&T5 & train & \asbar{0} & \asbar{1} & \asbar{0} & \asbar{96} & \asbar{93} & \asbar{100} & \asbar{85} \\ 
% \cmidrule{2-10}
&T5+aug & train & \asbar{100} & \asbar{1} & \asbar{0} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
&T5+aug+close brackets & train & \asbar{100} & \asbar{69} & \asbar{10} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
& Benepar & train100 & \asbar{84} & \asbar{95} & \asbar{98} & \asbar{99} & \asbar{100} & \asbar{100} & \asbar{99} \\
\midrule
\parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{pos}}} & BART & train & \asbar{0} & \asbar{5} & \asbar{21} & \asbar{84} & \asbar{85} & \asbar{100} & \asbar{85} \\
& T5 & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{73} & \asbar{78} & \asbar{100} & \asbar{83} \\
& T5+aug & train & \asbar{92} & \asbar{86} & \asbar{27} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{95} \\
% \midrule
% \parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{qa 1}}} & BART & train & \asbar{100} & \asbar{95} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
% \midrule
% \parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{qa 2}}} & BART & train & \asbar{68} & \asbar{53} & \asbar{63} & \asbar{63} & \asbar{89} & \asbar{100} & \asbar{86} \\
% & BART-QA & train & \asbar{90} & \asbar{68} & \asbar{100} & \asbar{86} & \asbar{91} & \asbar{100} & \asbar{94} \\
% \midrule
% \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{qa 3}}} & BART & train & \asbar{100} & \asbar{57} & \asbar{66} & \asbar{63} & \asbar{100} & \asbar{100} & \asbar{85} \\
% &T5 & train & \asbar{97} & \asbar{65} & \asbar{60} & \asbar{98} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
% & BART-QA & train & \asbar{100} & \asbar{96} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
\bottomrule
\end{tabular} 
    \caption{Exact match accuracies on the individual generalization types. We have compressed all 16 generalization types of the \lexg class into a single column and report the average accuracy. \todo{This table now need results from more seq2seq models like T5. Also now most results are based on train set rather than train100 so I need to run some BART experiments again. } \todo{Now the results in table 1 and table 2 are separate. I am also considering to merge them in one table but do not have a good idea on how to introduce them in the writing. }
    % \pw{to yuekun:}\yy{any updates from Z\&L re: per gen type results?}
    %Additionally to our own runs we copy numbers from \citet[Lex:Simple]{akyurek-andreas-2021-lexicon},  \citet[mT5 xl]{orhan-2021-compgen} and run own train100 experiments \yy{(1 run)} for \citet[\yy{model  config?}]{conklin-etal-2021-meta} and \citet[\yy{model  config?}]{csordas-etal-2021-devil}.
    }\label{tab:selected_gentype_eval}%\label{tab:selected_gentype_eval_transposed}
  \end{table*}

  
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> EMNLP 2022/tables/COGS_results_official.tex <==
\begin{table*}
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
\begin{tabular}{@{}lll|ccc|c|c@{}}
\toprule
& &  & \multicolumn{3}{c|}{\structg}  & \lexg & \\
& Model Class & Model & Obj to Subj PP & CP recursion & PP recursion & all 18 other types & Overall \\ 
\midrule
\multirow{11}{*}{semantics\qquad} 
& \multirow{9}{*}{seq2seq} & BART  & \asbar{0} & \asbar{0} & \asbar{12} & \asbar{91} & \asbar{79} \\
& & BART+syn  & \asbar{0} & \asbar{5} & \asbar{8} & \asbar{93} & \asbar{80} \\ 
& & T5  & \asbar{0} & \asbar{0} & \asbar{9}  & \asbar{97} & \asbar{83} \\ 
% &T5+aug & train & \asbar{0} & \asbar{64} & \asbar{46}  & \asbar{100} & \asbar{90} \\ 
% & &  \citealt{kim-linzen-2020-cogs}  & \asbar{0} & \asbar{0} & \asbar{0}  & \asbar{42} & \asbar{35} \\
& &  \citealt{kim-linzen-2020-cogs} & \asbar{0} & \asbar{0} & \asbar{0} &  \asbar{73} & \asbar{63} \\
& &  \citealt{akyurek-andreas-2021-lexicon}  & \asbar{0} & \asbar{0} & \asbar{1} & \asbar{96} & \asbar{82} \\
& &  \citealt{zheng-lapata-2022-disentangled}  & \asbar{0} & \asbar{12} & \asbar{39} & \asbar{99} & \asbar{89} \\
& & \citealt{conklin-etal-2021-meta} & \asbar{0} & \asbar{0} & \asbar{0} &\asbar{88} & \asbar{75} \\
& &  \citealt{csordas-etal-2021-devil} & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{95} & \asbar{81} \\
& &  \citealt{qiu2021improving} * & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} \\
\cmidrule[0.5pt]{2-8} 
& \multirow{2}{*}{\linf\qquad} & \citealt{liu-etal-2021-learning} & \asbar{93} & \asbar{100} & \asbar{99} & \asbar{99} & \asbar{99} \\ 
&  & \citealt{weissenhorn22starsem} & \asbar{78} & \asbar{100} & \asbar{99} & \asbar{100} & \asbar{98} \\ 
\midrule 
\multirow{3}{*}{syntax} & \multirow{2}{*}{seq2seq} & BART  & \asbar{0} & \asbar{9} & \asbar{22} & \asbar{99} & \asbar{87} \\
& &T5  & \asbar{5} & \asbar{7} & \asbar{9} & \asbar{99} & \asbar{86} \\ 
\cmidrule[0.5pt]{2-8} 
& \linf & Neural Berkeley Parser  & \asbar{84} & \asbar{95} & \asbar{98} & \asbar{100} & \asbar{99} \\
\midrule
\multirow{3}{*}{POS tags} & \multirow{2}{*}{seq2seq} & BART & \asbar{0} & \asbar{6} & \asbar{19}  & \asbar{98} & \asbar{85} \\
& & T5 & \asbar{0} & \asbar{4} & \asbar{4} & \asbar{98} & \asbar{85} \\ 
\cmidrule[0.5pt]{2-8} 
& \linf & most frequent POS  & \asbar{92} & \asbar{98} & \asbar{100} & \asbar{92} & \asbar{93} \\
% & T5+aug & train & \asbar{92} & \asbar{86} & \asbar{27} & \asbar{100} & \asbar{95} \\
% \midrule
% \parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{qa 1}}} & BART & train & \asbar{100} & \asbar{95} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
% \midrule
% \parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{qa 2}}} & BART & train & \asbar{68} & \asbar{53} & \asbar{63} & \asbar{63} & \asbar{89} & \asbar{100} & \asbar{86} \\
% & BART-QA & train & \asbar{90} & \asbar{68} & \asbar{100} & \asbar{86} & \asbar{91} & \asbar{100} & \asbar{94} \\
% \midrule
% \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{qa 3}}} & BART & train & \asbar{100} & \asbar{57} & \asbar{66} & \asbar{63} & \asbar{100} & \asbar{100} & \asbar{85} \\
% &T5 & train & \asbar{97} & \asbar{65} & \asbar{60} & \asbar{98} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
% & BART-QA & train & \asbar{100} & \asbar{96} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
\bottomrule
\end{tabular} 
    \caption{Exact match accuracies on the individual generalization types. 
    Column \lexg\ reports mean accuracy over the 18 lexical generalization types.
    *) After \linf\ data augmentation.
    }\label{tab:selected_gentype_eval}%\label{tab:selected_gentype_eval_transposed}
  \end{table*}

  
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> EMNLP 2022/tables/QA_results.tex <==
% \begin{table*}
%       \centering 
%       \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
%       \setlength{\tabcolsep}{2pt}
      
% \begin{tabular}{@{}ll|ccc|c|c@{}}
% \toprule
% &   & \multicolumn{3}{c|}{\structg}  & \lexg & \\
% Question & Model & Obj to Subj PP & CP recursion & PP recursion & all 18 other types & Overall \\ 
% % {\multirow{1}{*}{predicate classification}} & BART  & \asbar{100} & \asbar{95} & \asbar{100} & \asbar{100} & \asbar{99} \\
% \midrule
% {\multirow{3}{*}{argument identification}} & BART  & \asbar{68} & \asbar{53} & \asbar{63}  & \asbar{96} & \asbar{86} \\
% &T5  & \asbar{99} & \asbar{77} & \asbar{77}  & \asbar{97} & \asbar{94} \\ 
% & BART-QA  & \asbar{90} & \asbar{68} & \asbar{100} & \asbar{98} & \asbar{94} \\
% \midrule
% {\multirow{3}{*}{argument relation}} & BART  & \asbar{100} & \asbar{57} & \asbar{66} & \asbar{98} & \asbar{85} \\
% &T5  & \asbar{97} & \asbar{65} & \asbar{60} & \asbar{98} & \asbar{90} \\ 
% & BART-QA  & \asbar{100} & \asbar{96} & \asbar{100}  & \asbar{100} & \asbar{99} \\
% \bottomrule
% \end{tabular} 
%     \caption{Exact match accuracies on the individual generalization types on QA-COGS. 
%     % \todo{Need T5 number on qa2 set. I expect T5 could solve the PROP group.}
%     }\label{tab:qa_gentype_eval}%\label{tab:selected_gentype_eval_transposed}
%   \end{table*}


\begin{table*}[htbp!]
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
\begin{tabular}{@{}ll|ccc|c|c|c|c@{}}
\toprule
 & & \multicolumn{5}{c|}{\cogsqabase} & \multicolumn{2}{c}{\cogsqacc} \\
&   & \multicolumn{3}{c|}{\structg}  & \lexg & & & \\
Model Class & Model & Obj to Subj PP & CP recursion & PP recursion & all 18 other types & Overall & \textit{cc\_cp} & \textit{rc\_pp} \\ 
% {\multirow{1}{*}{predicate classification}} & BART  & \asbar{100} & \asbar{95} & \asbar{100} & \asbar{100} & \asbar{99} \\
\midrule
\multirow{2}{*}{seq2seq} & BART  & \asbar{99} & \asbar{59} & \asbar{69} & \asbar{95} & \asbar{86} & \asbar{37} & \asbar{14} \\
& T5  & \asbar{100} & \asbar{95} & \asbar{97} & \asbar{100} & \asbar{99} & \asbar{16} & \asbar{22} \\ \midrule
\multirow{2}{*}{\linf\qquad} & BART-QA  & \asbar{100} & \asbar{98} & \asbar{100}  & \asbar{100} & \asbar{99} & \asbar{6} & \asbar{0}\\
& BART-QA+struct\qquad\  & {-} & {-} & {-}  & {–} & {-} & \asbar{100} & \asbar{100}\\
\bottomrule
\end{tabular} 
    \caption{Exact match accuracy on the individual generalization types on the sections of \cogsqa.
    % \todo{Add annotations for seq2seq vs \linf\ as in Table 1.}
    % \todo{Need T5 number on qa2 set. I expect T5 could solve the PROP group.}
    }\label{tab:qa_gentype_eval}%\label{tab:selected_gentype_eval_transposed}
  \end{table*}


==> EMNLP 2022/tables/cogs_examples.tex <==
% \begin{table*}[htb!]
%     \small
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{\linewidth}{p{1.7cm}XX} \toprule
%          & \textbf{Training} & \textbf{Generalization} \\ \midrule
%          (a) \lexg
%          \newline {\tiny subj\_to\_obj}
%          \newline {\tiny (common noun)}
%          & {A \underline{hedgehog} ate the cake. \newline
%          \lform{*cake($x_4$); \underline{hedgehog($x_1$)} $\land$ eat.agent($x_2, \underline{x_1}$) $\land$eat.theme($x_2, x_4$)}} 
%          & {The baby liked the \underline{hedgehog}. \newline
%          \lform{*baby($x_1$); *\underline{hedgehog($x_4$)}; like.agent($x_2, x_1$) $\land$ like.theme($x_2, \underline{x_4}$)} }\\ 
%          \midrule
%          (b) \structg 
%          \newline {\tiny obj\_to\_subj PP}
%          & Ava saw a ball in a bowl on the table. \newline
%          \lform{*table($x_9$); see.agent($x_1,$ Ava) $\land$ see.theme($x_1, x_3$) $\land$ ball($x_3$) $\land$ ball.nmod.in($x_3, x_6$) $\land$ bowl($x_6$) $\land$ bowl.nmod.on($x_6,x_9$)}
%          &  Ava saw a ball in a bowl on the table \underline{on the floor}. \newline
%          \lform{*table($x_9$); \underline{*floor($x_{12}$);} see.agent($x_1,$ Ava) $\land$ see.theme($x_1, x_3$) $\land$ ball($x_3$) $\land$ ball.nmod.in($x_3, x_6$) $\land$ bowl($x_6$) $\land$ bowl.nmod.on($x_6,x_9$) \underline{$\land$ table.nmod.on($x_9,x_{12}$)}} \\ \cmidrule(l){2-3}
%          (c) \structg 
%          \newline {\tiny PP recursion} 
%          & Noah ate \underline{the cake on the plate}. \newline
%          \lform{*cake($x_3$); *plate($x_6$); \newline eat.agent($x_1,$ Noah) $\land$ eat.theme($x_1, x_3$) $\land$ cake.nmod.on($x_3,x_6$)} 
%          & \underline{The cake on the table} burned. \newline
%          \lform{*cake($x_1$); *table($x_4$); cake.nmod.on($x_1,x_4$) $\land$ burn.theme($x_3, x_1$)}\\ 
%          \bottomrule
%     \end{tabularx}
%     \caption{
%         Some examples from the COGS dataset. \lexg represent lexical generalization and \structg denotes structural generalization.
%     }\label{tab:cogssamples}
% \end{table*}


\begin{figure*}[htb!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{p{1.7cm}XX} \toprule
         & \textbf{Training} & \textbf{Generalization} \\ \midrule
         (a) \lexg
         \newline {\tiny subj\_to\_obj}
         \newline {\tiny (common noun)}
         & {A \underline{hedgehog} ate the cake. \newline
         \lform{*cake($x_4$); \underline{hedgehog($x_1$)} $\land$ eat.agent($x_2, \underline{x_1}$) $\land$eat.theme($x_2, x_4$)}} 
         & {The baby liked the \underline{hedgehog}. \newline
         \lform{*baby($x_1$); *\underline{hedgehog($x_4$)}; like.agent($x_2, x_1$) $\land$ like.theme($x_2, \underline{x_4}$)} }\\ 
         \midrule
         (b) \structg 
         \newline {\tiny PP recursion}
         & Ava saw a ball in a bowl on the table. \newline
         \lform{*table($x_9$); see.agent($x_1,$ Ava) $\land$ see.theme($x_1, x_3$) $\land$ ball($x_3$) $\land$ ball.nmod.in($x_3, x_6$) $\land$ bowl($x_6$) $\land$ bowl.nmod.on($x_6,x_9$)}
         &  Ava saw a ball in a bowl on the table \underline{on the floor}. \newline
         \lform{*table($x_9$); \underline{*floor($x_{12}$);} see.agent($x_1,$ Ava) $\land$ see.theme($x_1, x_3$) $\land$ ball($x_3$) $\land$ ball.nmod.in($x_3, x_6$) $\land$ bowl($x_6$) $\land$ bowl.nmod.on($x_6,x_9$) \underline{$\land$ table.nmod.on($x_9,x_{12}$)}} \\ \cmidrule(l){2-3}
         (c) \structg 
         \newline {\tiny obj\_to\_subj PP} 
         & Noah ate \underline{the cake on the plate}. \newline
         \lform{*cake($x_3$); *plate($x_6$); \newline eat.agent($x_1,$ Noah) $\land$ eat.theme($x_1, x_3$) $\land$ cake.nmod.on($x_3,x_6$)} 
         & \underline{The cake on the table} burned. \newline
         \lform{*cake($x_1$); *table($x_4$); cake.nmod.on($x_1,x_4$) $\land$ burn.theme($x_3, x_1$)}\\ 
         \bottomrule
    \end{tabularx}
    \caption{
        Some examples from the COGS dataset. \lexg represents lexical generalization and \structg denotes structural generalization.
    }\label{fig:cogssamples}
\end{figure*}

==> EMNLP 2022/tables/coordination_cp_example.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}


% \begin{table*}[]
%     \small
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{\linewidth}{X|X|X|X|X} \toprule
%         \multirow{2}{*}{Gen Type}& \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Generalization}} \\
%         % \hline
%         & \multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Question}}  & \multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Question}} \\
%         \hline
%         \multirow{3}{3.5cm}{\textit{cc\_cp}} & {Oliver liked that Noah discovers a boy } & {What did Oliver like?} & \multirow{3}{3cm}{Oliver liked that Noah discovers a boy and jogged . } & \multirow{3}{*}{What did Oliver like?} \\
%         & {Oliver slept and jogged} & {Who jogged?} & & \\
%         & {Oliver sleeps and jogs} & {Who jogs?} & & \\
%         \hline
%         \multirow{2}{3.5cm}{\textit{rc\_pp}} & {Olivia gave a box that was sketched to Benjamin} & { What was sketched?} & \multirow{2}{3cm}{Olivia gave a box in the houses that were sketched to Benjamin} & \multirow{2}{*}{What was sketched?} \\
%         & {Olivia gave boxes that were sketched to Benjamin} & {What was sketched?} & & \\
%          \bottomrule
%     \end{tabularx}
%     \caption{
%         Examples for our new generalization types. \textit{cc\_cp} denotes that we have complement clause and coordination structure separately during training and test their combination during generalization. \textit{rc\_pp} denotes that we have relative clause and preposition phrase structure separately during training and test their combination during generalization. 
%         % An example for combination of coordination structure and complement clause.
%         % \textcolor{red}{I reconsidered the \textit{cc\_cp} type and now I think the question we should ask in the test case is \textit{Who jogged?} rather than \textit{What did Oliver like?} }
%         % bold? underline? colors?
%     }\label{tab:coordination_cp_example}
% \end{table*}



==> EMNLP 2022/tables/probe_results.tex <==
\begin{table}
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
\begin{tabular}{@{}lll|ccc|c@{}}
\toprule
& &  & \multicolumn{3}{c|}{\structg} & \lexg \\
& Encoder & Data & Obj to Subj PP & CP recursion & PP recursion  & all 18 other types  \\ 
\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{sem}}} 

& BART & probe & \asbar{82} & \asbar{91} & \asbar{92}  & \asbar{100}  \\
& Random & probe & \asbar{25} & \asbar{0} & \asbar{65}  & \asbar{90}  \\
& BART & orig & \asbar{0} & \asbar{5} & \asbar{27} & \asbar{94} \\
% & Random & probe & \asbar{1} & \asbar{0} & \asbar{0} & \asbar{34} & \asbar{40} & \asbar{10} & \asbar{14} \\
\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{syn}}} & BART & probe & \asbar{85} & \asbar{80} & \asbar{83} & \asbar{100}  \\
% \cmidrule{2-10}
& Random & probe & \asbar{1} & \asbar{0} & \asbar{0}  & \asbar{16}  \\
& BART & orig & \asbar{0} & \asbar{0} & \asbar{7} & \asbar{92} \\
% & Random & probe & \asbar{27} & \asbar{1} & \asbar{61} & \asbar{92} & \asbar{93} & \asbar{90} & \asbar{82} \\
\bottomrule
\end{tabular} 
    \caption{Exact match accuracy for probing on the individual generalization types. 
    }\label{tab:probe_eval}%\label{tab:selected_gentype_eval_transposed}
  \end{table}

  
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> EMNLP 2022/tables/qa_cogs_examples.tex <==
\begin{table*}[htb!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|X|X|X} \toprule
         \textbf{Predicate Frame} & \textbf{Context} & \textbf{Question} & \textbf{Answer} \\ 
         \midrule
         {\genclass{agent}} & {The captain ate}  & {Who ate ?} & {the captain}\\
         \midrule
         {\genclass{theme}} & {The donut was known}  & {What was known ?} & {the donut}\\
         \midrule
         \multirow{2}{*}{\genclass{agent\_theme}} & \multirow{2}{3cm}{Emma ate the ring beside a bed}  & {What did Emma eat. ?} & {the ring beside a bed} \\
         & & {Who ate the ring beside a bed ?} & {Emma} \\   
         \midrule
         \multirow{3}{*}{\genclass{agent\_theme\_recipient}} & \multirow{3}{3cm}{Amelia gave Emma a strawberry}  & {Who gave a strawberry to Emma ?} & {Amelia} \\
         & & {What did Amelia give to Emma ?} & {a strawberry} \\
         & & {Who did Amelia give a strawberry to ?} & {Emma} \\
         \midrule
         \multirow{2}{*}{\genclass{theme\_recipient}} & \multirow{2}{3cm}{A rose was mailed to Isabella}  & {Who was a rose mailed to ?} & {Isabella}\\
         & & {What was mailed to Isabella ?} & {a rose} \\
         \midrule
         \multirow{2}{*}{\genclass{agent\_ccomp}} & \multirow{2}{3cm}{Liam meant that Sophia  rolled a teacher on a seat}  & {What did Liam mean ?} & {that Sophia rolled a teacher on a seat} \\
         & & {Who meant that Sophia rolled a teacher on a seat ?} & {Liam} \\
         \midrule
         \multirow{2}{*}{\genclass{agent\_xcomp}} & \multirow{2}{*}{Emma hoped to run}  & { Who hoped to run ?} & {Emma}\\
         & & {What did Emma hope to do ?} & {run} \\
         \bottomrule
    \end{tabularx}
    \caption{
        All possible predicate frames and corresponding question-answer examples for the QA-COGS-base dataset.
        % bold? underline? colors?
    }\label{tab:qacogssamples}
\end{table*}



% \begin{table*}[htb!]
%     \small
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{\linewidth}{l|l|X|X|X} \toprule
%          & \textbf{Predicate Frame} & \textbf{Context} & \textbf{Question} & \textbf{Answer} \\ 
%          \midrule
%          \multirow{2}{*}{\textbf{Predicate Classification}} & \multirow{1}{*}{\genclass{agent\_theme}} & \multirow{1}{3.3cm}{Emma ate the ring beside a bed}  & {Which arguments does \textit{eat} take?} & {agent theme} \\
%         %  \midrule
%          & \multirow{1}{*}{\genclass{agent\_ccomp}} & \multirow{1}{3.3cm}{Liam meant that Sophia  rolled a teacher on a seat}  & {Which arguments does \textit{mean} take?} & {agent ccomp} \\
%          \midrule
%          \multirow{4}{*}{\textbf{Argument Identification}} & \multirow{2}{*}{\genclass{agent\_theme}} & \multirow{2}{3.3cm}{Emma ate the ring beside a bed}  & {What is the \textit{theme} of \textit{eat}?} & {the ring beside a bed} \\
%          & & & {What is the \textit{agent} of \textit{eat}?} & {Emma} \\   
%         %  \midrule
%          & \multirow{2}{*}{\genclass{agent\_ccomp}} & \multirow{2}{3.3cm}{Liam meant that Sophia  rolled a teacher on a seat}  & {What is the \textit{ccomp} of \textit{mean}?} & {that Sophia rolled a teacher on a seat} \\
%          & & & {What is the \textit{agent} of \textit{mean}?} & {Liam} \\
%          \midrule
%          \multirow{4}{*}{\textbf{Argument Relation}} & \multirow{2}{*}{\genclass{agent\_theme}} & \multirow{2}{3.3cm}{Emma ate the ring beside a bed}  & {What did Emma eat. ?} & {the ring beside a bed} \\
%          & & & {Who ate the ring beside a bed ?} & {Emma} \\   
%         %  \midrule
%          & \multirow{2}{*}{\genclass{agent\_ccomp}} & \multirow{2}{3.3cm}{Liam meant that Sophia  rolled a teacher on a seat}  & {What did Liam mean ?} & {that Sophia rolled a teacher on a seat} \\
%          & & & {Who meant that Sophia rolled a teacher on a seat ?} & {Liam} \\
%          \bottomrule
%     \end{tabularx}
%     \caption{
%         Some examples for the QA-COGS dataset. 
%         % \todo{It is good to relate these sentences to COGS gen type but I do not know how to do this properly.}
%         % bold? underline? colors?
%     }\label{tab:qacogssamples}
% \end{table*}

==> EMNLP 2022/tables/qa_detailed_results.tex <==
\begin{table}[]
    \small
    \centering
\begin{tabular}{lcc}
Type & BART & BART-QA \\ \midrule
Subj to Obj (common noun) & 100 & 100\\
Subj to Obj (proper noun) & 100 & 100 \\
Obj to Subj (common noun) & 100  & 100 \\
Obj to Subj (proper noun) & 100 & 100  \\ 
\midrule
Prim to Subj (common noun) & 100 & 100 \\
Prim to Subj (proper noun) & 96 & 100 \\
Prim to Obj (common noun) & 100 & 100 \\
Prim to Obj (proper noun) & 63 & 100 \\
Prim verb to Infin. arg & 55 & 100 \\
\midrule
ObjmodPP to SubjmodPP & 100 & 100 \\
CP recursion & 57 & 96  \\
PP recursion & 66 & 100 \\
\midrule
Active to Passive & 100 & 100 \\
Passive to Active & 100 & 100 \\
ObjOTrans. to trans. & 100 & 100 \\
Unacc to transitive & 100 & 100 \\
Dobj dative to PP dative & 100 & 100 \\
PP dative to Dobj dative & 100 & 100 \\ 
\midrule
Agent NP to Unacc Subj & 100  & 100\\
Theme NP to ObjOTrans. Subj & 100 & 100 \\
Theme NP to Unergative Subj & 100 & 100 \\ 
\midrule
Total & 85 & 99\\
\bottomrule
    \end{tabular}
    \caption{
        Exact match accuracy on the generalization set by generalization type
        \todo{We may need more columns for T5, LSTM and transformers (without pretraining). In that case, maybe it's better to changed this table into the format we used in the reject paper?}
    }\label{tab:qa_detailed_results}
\end{table}

==> EMNLP 2022/tables/qa_gen_examples.tex <==
% \begin{table*}[htb!]
%     \small
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{\linewidth}{ll|X|X}
%         \toprule
%       & & \textbf{Training}  &  \textbf{Generalization} \\
%       \toprule
%         \multirow{3}{*}{Obj to Subj PP} & Context & {Noah ate the cake on the plate} & {The cake on the plate burned}\\ 
%         & Question & {{What did Noah eat?}} & {What was burned?} \\ 
%         & Answer & {\lform{the cake on the table}} & {\lform{the cake on the plate}} \\ 
%         \midrule
%         \multirow{3}{*}{PP recursion} & Context & {Ava saw a ball in a bowl on the table} & {Ava saw a ball in a bowl on the table on the floor} \\ 
%         & Question & {{What did Ava see?}} & {What did Ava see?} \\ 
%         & Answer & {\lform{a ball in a bowl on the table}} & { \lform{a ball in a bowl on the table on the floor }}\\ 
%         \midrule
%         \multirow{3}{*}{CP recursion} & Context & {Ava said that Emma liked that a dog ran.} & {Ava said that Emma liked that Noah noticed that a dog ran.} \\ 
%         & Question & {{What did Ava say?}} & {What did Ava say?} \\ 
%         & Answer & {\lform{that Emma liked that a dog ran}} & { \lform{that Emma liked that Noah noticed that a dog ran}}\\
%         \bottomrule

%     \end{tabularx}
%     \caption{Examples for QA-COGS with regard to each structural generalization type.}
%     \label{tab:qa_gen_examples}
% \end{table*}



\begin{figure*}[htbp!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{lXX}
        \toprule
        \textbf{Gen type} & \textbf{Training}  &  \textbf{Generalization} \\
       \midrule
    %   \multicolumn{3}{c}{Argument Relation Sec \ref{para:arg_relation}} \\
    %   \midrule
        {Obj to Subj PP}  & {Noah ate  {\textbf{the cake on the plate}}. What did Noah eat?} & { {\textbf{The cake on the plate}} burned. What was burned?}\\ 
        \midrule 
        {PP recursion}  & {Ava saw {\textbf{a ball in a bowl on the table}}. What did Ava see?} & {Ava saw  {\textbf{a ball in a bowl on the table on the floor}}. What did Ava see?} \\ 
        \midrule
        {CP recursion}  & {Ava said  {\textbf{that Emma liked that a dog ran}}. What did Ava say?} & {Ava said  {\textbf{that Emma liked that Noah noticed that a dog ran}}. What did Ava say?} \\ 
        % \midrule
        % \multicolumn{3}{c}{Argument Identification Sec \ref{para:arg_identification}} \\ 
        % \midrule
        % {Obj to Subj PP}  & {Noah ate \textbf{{the cake on the plate}}. What is the \textit{theme} of \textit{ate}?} & { \textbf{{The cake on the plate}} burned. What is \textit{agent} of \textit{burned}?}\\ 
        % \midrule
        % {PP recursion}  & {Ava saw {\textbf{a ball in a bowl on the table}}. What is the \textit{theme} of \textit{saw}?} & {Ava saw {\textbf{a ball in a bowl on the table on the floor}}. What is the \textit{theme} of \textit{saw}?} \\ 
        % \midrule
        % {CP recursion}  & {Ava said {\textbf{that Emma liked that a dog ran}}. What is the \textit{ccomp} of \textit{said}?} & {Ava said {\textbf{that Emma liked that Noah noticed that a dog ran}}. What is the \textit{ccomp} of \textit{said}?} \\ 
        \bottomrule

    \end{tabularx}
    \caption{Examples for the \cogsqabase\  dataset with regard to each structural generalization type. In each example, the first sentence is the context sentence, the second sentence is the question sentence and the bold token span is the corresponding answer.}
    \label{fig:qa_gen_examples}
\end{figure*}


==> EMNLP 2022/tables/qa_prim_error_examples.tex <==
\begin{table*}[htb!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|X|X|X|X} \toprule
         \textbf{generalization types} & \textbf{Context} & \textbf{Question} & \textbf{Gold} & Pred\\ 
         \midrule
         \textit{prim\_to\_subj\_proper} & {Noah imagined that Emma supported that Paula wanted to dance .}  & {Who did Noah imagine that Emma support that want to dance ?} & {Paula} & {Paula Paula}\\
         \midrule
        \textit{prim\_to\_obj\_proper} & {Evelyn gave Paula to a journalist .} & {What did Evelyn give to a journalist ?} & {Paula} & {Paula Paula} \\
        \midrule
        \textit{prim\_to\_inf\_arg} & {The consumer hated to crawl .} & {What did the consumer hate to do ?} & {crawl} & {crawl crawl} \\
        % \midrule
        % \textit{obj\_pp\_to\_subj\_pp} & {The baby on a tray in the house screamed .} & {Who screamed ?} & {the baby on a tray in the house} & {the baby on a tray in the house} \\
         \bottomrule
    \end{tabularx}
    \caption{
        Some examples for the QA-COGS dataset.
        % bold? underline? colors?
    }\label{tab:qa_prim_error_examples}
\end{table*}

==> EMNLP 2022/tables/rc_example.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{lXX} \toprule
Context & \textit{Emma ate the rings beside a bed that \textcolor{red}{was} called} & \textit{Emma ate the rings beside a bed that \textcolor{red}{were} called} \\
\midrule
Gold &  \textit{a bed} & \textit{the rings beside a bed}\\
BART &  \textit{the rings beside a bed} & \textit{the rings beside a bed} \\
BART-QA &  \textit{the rings beside a bed} & \textit{the rings beside a bed} \\
 \bottomrule
\end{tabularx}
\caption{Error example for BART and BART-QA. In this sentence the question is \textit{What was called?}}\label{tab:error_rc}
\end{table}


==> EMNLP 2022/tables/struct_gen_type_results.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}{ccccccccccc}
%     \multirow{2}{*}{ Model } & \multicolumn{5}{c}{rc\_pp} & \multicolumn{5}{c}{cc\_cp} \\
%     & sg\_pl & sg\_sg & pl\_sg & pl\_pl & avg & ps\_pr & ps\_ps & pr\_ps & pr\_pr & avg \\
%     BART & 14 & 80 & 2 & 96 & 48 & 1 & 100 & 1 & 100 & 51 \\
%     BART-QA & 6 & 85 & 0 & 100 & 48 & 48 & 74 & 62 & 85 & 67 \\    \end{tabular}
%     \caption{exact accuracy on new test set }
%     \todo{I plan to change the coordination experiments so will update this table after that. }

%     \label{tab:qa_struct_results}
% \end{table*}

\begin{table}[]
    \centering
    \begin{tabular}{c|cc}
    Model & rc\_pp & cc\_cp \\
    \toprule
    BART & 48 & 51 \\
    BART-QA & 48 & 67 \\
    BART-QA+syn & - & 100 \\
    \bottomrule
    \end{tabular}
    \caption{exact accuracy on new test set }
    % \todo{I plan to change the coordination experiments so will update this table after that. }

    \label{tab:qa_struct_results}
\end{table}

==> sections/Experiment.tex <==
\section{Experiments}

\subsection{setup}
\paragraph{QA setup} \label{subsec:seq2seq:setup}
We train BART as our model on QA-COGS.  To apply BART for the question answering task, we directly fine-tune the pretrained \textit{bart-base} model on it with the corresponding tokenizer. During fine-tuning, the model takes as input the concatenation of context and question strings and outputs the answer.

We also had another model named BART-QA for comparison. BART-QA simply applies two multi-layer perceptrons over the hidden states from BART to determine the start and end index of a span in the context. The selected span is used as the predicted answer. 

% \paragraph{\textcolor{red}{which other models should we use for experiments}}If the focus of the whole story is  \textit{seq2seq models fail on compgen}, we should also use LSTM (with copy mechanism) and perhaps GRU. If the focus is \textit{compgen on text-to-text generation tasks}, we should also give some space for extract question answering model.

\subsection{results}

Table \ref{tab:selected_gentype_eval} shows the results of our models on QA-COGS. We can observe that seq2seq models solve the predicate classification task, but still struggle on argument identification and relation tasks. We thus focus on discussing these results on these two tasks.

% \input{tables/qa_detailed_results}

\paragraph{Lexical Generalization} We first look at argument relation task. Clearly, seq2seq solves most lexical generalization types except for \textit{prim\_to\_subj\_proper}, \textit{prim\_to\_obj\_proper} and \textit{prim\_to\_inf\_arg}. Looking into the output of the model, we find that errors for such primitive generalization types all come from the inability to copy the primitive as seen below. 
\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{Noah imagined that Emma supported that Paula wanted to dance .}
    
    \textbf{Question} \textit{Who did Noah imagine that Emma support that want to dance ?}
    
    \textbf{Gold} \textit{Paula}
    
    \textbf{Pred} \textit{Paula Paula}
    
    }
}
\end{center}

Note that a primitive in original COGS is only annotated as either its word form or a lambda expression, so we cannot generate question-answer pairs for primitives in the train set. This means that such primitives (e.g. \textit{Paula} and \textit{crawl}) are out-of-vocabulary tokens for our model. We consider such errors are mainly due to the instability of fine-tuning our pretrained seq2seq models. \textcolor{red}{We should also use seq2seq with copy mechanism to get a better picture here.} However, another question exists: why the model can meanwhile solve the common noun cases (e.g. \textit{prim\_to\_obj\_common})? Does BART have some internal weakness for proper nouns? We currently do not have a clear answer for this. \textcolor{red}{ T5 does not have this issue so maybe this paragraph does not make much sense and we can just say it's the internal weakness of BART. Of course we can replace \textit{Paula} in the generalization set with other proper nouns to confirm this assumption.} T5 and extractive model perform well on this type. 

Now look at the argument relation task. Both extractive and seq2seq models cannot fully solve \textit{prim\_to\_obj\_proper}. However, we notice that for the same sentence, the two models make different types of errors as seen in the example below. \todo{Maybe I should add primitive word into the train set or try T5 on this task. This discussion does not make much sense to myself.} If extractive model cannot recognize Paula as a theme, how could it solve the argument relation task? Noticing that in relation task the question will become \textit{What did Emma sell the girl?}, we consider the extractive model simply learns to select the span not occurring in the question string. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{Emma sold the girl Paula .}
    
    \textbf{Question} \textit{What is the theme of sell ?}
    
    \textbf{Gold} \textit{Paula}
    
    \textbf{BART Pred} \textit{the girl}
    
    \textbf{BART-QA Pred} \textit{the girl Paula}
    
    }
}
\end{center}

\paragraph{obj\_pp\_to\_subj\_pp} Still we first look at the argument relation task. Different from the COGS result, seq2seq models performs well on \textit{obj\_pp\_to\_subj\_pp} type. Does this mean seq2seq model learns to combine PP structure with any nouns? Notice that to give the correct answer in the example below, the model can simply copy the context string on the left of the predicate word (e.g. screamed). Thus, this type is not enough to evaluate the ability to learn structure. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{ The baby on a tray in the house screamed .}
    
    \textbf{Question} \textit{ Who screamed ?}
    
    \textbf{Gold} \textit{ the baby on a tray in the house}
    
    \textbf{Pred} \textit{ the baby on a tray in the house}
    
    }
}
\end{center}

On the other hand, both seq2seq and extractive models does not solve this type in argument identification task. We find the main reason for this error is that both models possibly ignore the prepositional phrase modifying the subject as seen below. \todo{This actually could be counted as correct, though I do not know if this makes much sense.}
\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{A donkey in the room sold Ella a donut .}
    
    \textbf{Question} \textit{What is the agent of sell ?}
    
    \textbf{Gold} \textit{a donkey in the room}
    
    \textbf{BART Pred} \textit{a donkey}
    
    \textbf{BART-QA Pred} \textit{a donkey}
    
    \textbf{Question} \textit{What is the theme of sell ?}
    
    \textbf{Gold} \textit{a donut}
    
    \textbf{BART Pred} \textit{a donut in the room}
    
    \textbf{BART-QA Pred} \textit{a donut}
    
    }
}
\end{center}

\paragraph{recursion types} For CP and PP recursion types on relation task, our result is consistent with the pattern in semantic parsing. An error example for CP recursion is listed below. 

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{ Aiden liked that Liam liked that Avery appreciated that the dog expected that a cat liked that Emma appreciated that a donut was loved .}
    
    \textbf{Question} \textit{ What did Aiden like that Liam like?}
    
    \textbf{Gold} \textit{ that Avery appreciated that the dog expected that a cat liked that Emma appreciated that a donut was loved}
    
    \textbf{Pred} \textit{ that Avery appreciated that the dog expected that a cat liked that a cat liked that a cat.....}
    
    }
}
\end{center}

Again, such questions can be solved by simply generating the context string on the left of \textit{...that Liam like}. However, our result indicates that the seq2seq model does not even learn this simple heuristic. We also plot the result of our model with regard to answer recursions and context recursions for CP\_recursion typed sentences in Fig \ref{fig:qa_depth}. We can observe that for all depths of contexts, the performance always decreases as the answer depth grows. This is consistent with previous findings that seq2seq struggles on generating longer sequence than it sees during training, since our train set only contains sentences with at most 2 CP recursions. Another observation is that, for the same answer depth, larger context depth gives lower performance. However, this does not hold for answer depth 1 and 2, where the model performs well on cd=11-12 but worse on cd=6-8. We do not a good explanation about this for now. 
 
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/qa_recursion_depth.pdf}
    \caption{Exact match accuracy of BART on CP recursion typed questions. Answer depth denotes the number of CP recursions in the answer and \textit{cd} denotes the number of CP recursions in the context. \textcolor{red}{Need to make this figure easier to read.}}
    \label{fig:qa_depth}
\end{figure}

For identification task, seq2seq still struggle on both types. Interestingly, extractive models could solve \textit{pp\_recursion} but cannot solve \textit{cp\_recursion}. An example is shown below. We currently do not know why this happens.

\begin{center}
\noindent\fbox{
    \parbox{.9\linewidth}{
    \textbf{Context} \textit{A girl valued that Samuel admired that a monkey liked that Luna liked that Oliver respected that Savannah hoped that a penguin noticed that Emma noticed that the lawyer noticed that a cake grew .}
    
    \textbf{Question} \textit{ What is the agent of respect ?}
    
    \textbf{Gold} \textit{Oliver}
    
    \textbf{BART-QA Pred} \textit{Samuel}
    
    }
}
\end{center}

% \input{tables/qa_prim_error_examples}

% \paragraph{\textcolor{red}{Are we learning heuristics rather than compositionality?}} I feel that what I can say in this section is very shallow and I am now very worried that our model learns a lot of heuristics rather than compositionality to solve QA-COGS. Most examples in Table \ref{tab:qacogssamples} can be solved by some simple heuristics (e.g. output part of the context string which does not appear in the question string) rather than compositional generalization. If model only learns such heuristics, then this corpus really does not make any sense. 

% For example, for \textit{unacc\_to\_transitive} generalization type, we only have one sample in the train set below:

% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ Julian shattered .}
    
%     \textbf{Question} \textit{ What was shattered ?}
    
%     \textbf{Gold} \textit{ Julian}
    
%     \textbf{MR} \textit{ shatter . theme ( x \_ 1 , Julian )}
    
%     }
% }
% \end{center}

% % \textit{Context: Julian shattered .}

% % \textit{Q: What was shattered ?}

% % \textit{gold: Julian}

% % \textit{MR:  shatter . theme ( x \_ 1 , Julian )}

% and then in the generalization set we have:

% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The cat shattered the cake .}
    
%     \textbf{Question} \textit{ What did the cat shatter ?}
    
%     \textbf{Gold} \textit{ the cake}
    
%     \textbf{MR} \textit{ * cat ( x \_ 1 ) ; * cake ( x \_ 4 ) ; shatter . agent ( x \_ 2 , x \_ 1 ) AND shatter . theme ( x \_ 2 , x \_ 4 )}
    
%     }
% }
% \end{center}

% In semantic parsing task this makes sense, but in QA-COGS this task becomes too simple and can be solved by not using compositionality. This issue almost holds for all lexical generalization types, so we really should address this. 

% Another question I am considering is to ask different questions. Remember that the motivation of bAbI is to evaluate different reading comprehension abilities of neural models through a lot of toy tasks. (Our corpus is actually the task 5 \href{https://arxiv.org/pdf/1502.05698.pdf}{here}). As I mentioned in section \ref{sec:overview}, we can similarly split COGS into multiple tasks and evaluate them independently. As I can imagine, to solve COGS we need at least four abilities: 1) the ability to recognize the frame of a predicate 2) the ability to find the argument for a predicate 3) the ability to differentiate common nouns and proper nouns 4) the ability to count the index of a token. Our current corpus only tests the ability (2), so can we also test other abilities by asking new questions? 

% For example, to test ability (1), we can have questions like below:
% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The cat shattered the cake .}
    
%     \textbf{Question} \textit{ Which arguments does \textit{shatter} take ?}
    
%     \textbf{Gold} \textit{ agent theme}
    
%     }
% }
% \end{center}
% Such questions may also give us a better picture about whether our model learns heuristic or compositionality. 

% To test the ability (3), we may have:
% \begin{center}
% \noindent\fbox{
%     \parbox{.9\linewidth}{
%     \textbf{Context} \textit{ The captain ate.}
    
%     \textbf{Question} \textit{ What is the index of \textit{captain}?}
    
%     \textbf{Gold} \textit{ 1}
    
%     }
% }
% \end{center}
% If the model cannot even solve this task for recursion types in the generalization set, it indicates that the failures of seq2seq on recursion generalization in COGS may be due to the counting inability.

==> sections/New_generalization_types.tex <==

\section{Structural generalization without length generalization}
% \todo{Maybe this section could just be a subsection of QA-COGS. I do not think we say more beyond \textit{seq2seq and extractive models still fail on struct generaliation on QA.}}
We have seen the generalization set of QA-COGS has some limitations: the Obj to Subj PP type tests shallow compositionality while recursion types only tests length generalization ability. It is still unclear whether structural generalization is difficult or not when disentangled from length generalization. To explore this question, we create two new QA  datasets named \textit{cc\_cp} and\textit{rc\_pp} and observe model behaviours on these new datasets.

We start by introducing \textit{cc\_cp} corpus. The idea of this dataset is to test whether the model can generalize to unseen combination of the coordination structure(\textit{cc}) and the complement clause(\textit{cp}). An example is shown in the \textit{cc\_cp} row in Table \ref{tab:coordination_cp_example}. During training, the model sees context sentences with either a coordination structure (e.g. \textit{sleeps and jogs}) or a complement clause (e.g.  \textit{liked that Noah discovers a boy}), but never observes their combination in one context sentence. In the generalization set, we combine these two structures into one context sentence(e.g. \textit{liked that Noah discovers a boy and jogged}) and ask the question \textit{What did Oliver like?}. To answer this correctly, the model needs to be aware that verb tenses inside the coordination structure should be the same, and thus verb tenses determine whether the last verb(e.g. jog) should be coordinated with the verb inside the complement clause(e.g. discover) or outside the complement clause(e.g. like). 

Similarly, we test the combination of the relative clause structure(\textit{rc}) and the prepositional phrase structure(\textit{pp}) in \textit{rc\_pp}. The example is shown in the \textit{rc\_pp} row in Table \ref{tab:coordination_cp_example}. In this dataset we make the model learn \textit{rc}(e.g. \textit{boxes that were sketched}) and \textit{pp}(e.g. \textit{boxes in the house}) structure separately, and test their combination(e.g. \textit{boxes in the house that was sketched}) with the question \textit{What was sketched?}. To answer this correctly, the model needs to learn whether \textit{rc} modifies the noun inside \textit{pp} or outside \textit{pp} based on its verb form(e.g. \textit{was/were}).

Now we describe how we create such datasets in practice. For \textit{cc\_cp}, the train set consists of \textit{cp} sentences and \textit{cc} sentences. For \textit{cp} sentences, we directly copied from the original QA-COGS train set. For \textit{cc} sentences, we randomly sample 2000 sentences(without \textit{cp} structure) from  original QA-COGS train set and adding an unergative verb to the sampled sentences. The generalization set is then generated with a hand-written heuristic based on each \textit{cp} sentence in the train set. As shown in Figure \ref{fig:struct_example}, each \textit{cp} sentence in the train set will result in 4 sentences in generalization set. For\textit{rc\_pp}, the train set consists of \textit{rc} sentences and \textit{pp} sentences. We still obtain \textit{pp} sentences by copying from original QA-COGS and generate \textit{rc} sentences by adding a random relative clause into 2000 sampled QA-COGS sentences. The \textit{rc} is generated by using a random passive verb(e.g.\textit{ that was painted}). The generalization set for \textit{rc\_pp} is then generated by a heuristic similar to \textit{cc\_cp}. Our generated sentences share the same vocabulary with original COGS sentences and we control all clauses depth always being 1, so there is no length generalization in our datasets. 
% The train set of \textit{cc\_cp} consists of two parts. The first part is copied exactly from the original train set of QA-COGS. The second part 

% Noticing that current questions are not enough to test the structural generalization for compositionality, we extend the corpus with two new structural generalization types, named as \textit{cc\_cp} and \textit{rc\_pp}. Specifically, we introduce relative clause and coordination structures into the train set of QA-COGS and test their combination with prepositional phrase and complement clause respectively. 
% In addition to the questions we described in section \ref{sec:overview}, we also introduce coordination structure into our train set and combine the coordination structure with complement clause in the generalization set. 
\input{tables/coordination_cp_example} 

% An example of our idea can be seen in Table \ref{tab:coordination_cp_example}. For \textit{cc\_cp} type, a compositionality-aware model should be able to learn that the predicate \textit{jog} in the generalization example should be coordinated with \textit{like} according to the tense, and thus the answer will be \textit{that Noah discovers a boy}. However, a model that does not learn structural generalization will possibly answer \textit{that Noah discovers a boy and jogged}. Similarly, in \textit{rc\_pp}, the form of \textit{be} verb (i.e. \textit{was/were}) determines which noun is attached by the prepositional phrase, but a heuristic-based model cannot learn this. 

% To create test data for \textit{cc\_cp}, for a sentence containing complement clause in the original train set, we randomly sample an unergative verb and combine them with a coordination structure. An example can be seen in the first case of Figure \ref{fig:struct_example}. Note that to obtain an unambiguous sentence, we need to guarantee the main verb has a different tense from the clause verb(i.e. \textit{Oliver liked that Noah discovered a boy and jogged} is ambiguous). Thus, depending on the combination of tenses of main verb and clause verb, we generate 4 sentences for each original COGS sentence as our new test set. To create the train set, we randomly sample 2000 sentences without complement clauses from the original train set and add coordination structure to the sampled sentences. We then concatenate resulted sentences with original train set as new train set.  

% To create test data for \textit{rc\_pp}, for a sentence containing preposition phrase in the original train set, we randomly sample a verb that takes a noun as the argument and combine them with a relative clause. An example can be seen in the second case of Figure \ref{fig:struct_example}. Similar to the \textit{cc\_cp} case, we need to guarantee two nouns have different singular and plural forms and thus obtain 4 sentences for each original COGS sentence as our new test set. We also introduce relative clauses into 2000 sentences without prepositional phrase in the original train set and concatenate them as new train set. 

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figures/struct_example.png}
    \caption{Example of generating generalization data for \textit{rc\_cc} and \textit{cc\_cp}.}
    \label{fig:struct_example}
\end{figure}

% \todo{introduce how to create the dataset}

\subsection{Experiment Setup}

In addition to the models introduced in section \ref{subsec:seq2seq:setup}, we also train a syntax-aware BART-QA model named \textit{BART-QA+syn} to make comparison. Instead of selecting an arbitrary span from the context string, this syntax-aware model is given the gold constituent tree and then constrained to select a constituent span for both training and inference. 

\subsection{Results}

\input{tables/struct_gen_type_results}

The results are shown in Table \ref{tab:qa_struct_results}. We observe BART-QA now fails on these two new generalization dataset. We consider this is because different from the structural generalization types in section \ref{sec:overview}, our new datasets can not be solved by a string-level heuristic. For BART, our dataset is still difficult. Note that since we only have recursion depth being 1 in our new test data, this difficulty genuinely comes from the structural generalization rather than length generalization.  
% indicating the inability of seq2seq models to combine known structures. 
However, BART-QA+syn achieves great accuracy, which means that a syntax-aware model is robust in structural generalization. 

\input{tables/rc_example}

Looking into the output of BART and BART-QA, we find both models tend to output the same span with different \textit{be} verb forms as shown in Table \ref{tab:error_rc}. We consider this is because models without structure bias directly learn to select the span on the left of the relative clause. 

% We apply the same models as in section \ref{subsec:seq2seq:setup} on our new corpuses. 
% The results is shown in Table \ref{tab:qa_struct_results}. Note that our introduced structure (e.g. coordination structure) could be attached to the verb either in the main sentence or the clause. We report the accuracy for the two categories separately as \textbf{main} and \textbf{sub}. 

% \todo{Remember we have many possible splits for \textit{cc\_cp}.  Which setting and results should we present here? }

% \todo{I found that when we test BART model on \textit{cc\_cp} type, the model always outputs the complement clause without the coordination structure. Maybe it is because our training samples do not contain \textbf{\textit{and}} in the output side. I now plan to change the questions for cc\_cp type to avoid this problem. I will finish this section after that. }

% \paragraph{results} To be updated.
% \todo{Introduce the extractive model }

% \paragraph{\textcolor{red}{Connection with extractive model}} We have spent much efforts on exploring performance of extractive models on QA-COGS. However, I am now very confused on how to connect that work with the current story. I developed the extractive model because our initial story is to present a QA corpus, and thus we need to experiment with seq2seq, extractive and structured models. If our story now is \textit{seq2seq is not good at compgen}, then why do we need to present results of extractive models in this story?


==> tables/COGS_results.tex <==
\begin{table*}
      \centering 
      \scriptsize % \tiny \scriptsize \footnotesize \small \normalsize
      \setlength{\tabcolsep}{2pt}
      
\begin{tabular}{@{}lll|ccc|cc|c|c@{}}
\toprule
& & Class & \multicolumn{3}{c|}{\structg} & \multicolumn{2}{c|}{\propg} & \lexg & \\
& & Gen. type & Obj to Subj PP & CP recursion & PP recursion & prim to
                                                               obj
                                                               (proper)
  & subj to obj (proper) & all 16 other types & Overall \\ 
\midrule
\parbox[t]{1mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{sem}}} 

& BART & train100 & \asbar{0} & \asbar{0} & \asbar{10} & \asbar{55} & \asbar{86} & \asbar{99} & \asbar{83} \\
& BART+syn & train100 & \asbar{0} & \asbar{7} & \asbar{8} & \asbar{98} & \asbar{95} & \asbar{100} & \asbar{86} \\ 
&T5 & train & \asbar{0} & \asbar{0} & \asbar{5} & \asbar{71} & \asbar{70} & \asbar{100} & \asbar{83} \\ 
&T5+aug & train & \asbar{0} & \asbar{64} & \asbar{46} & \asbar{89} & \asbar{89} & \asbar{100} & \asbar{90} \\ 
& LeAR & train & \asbar{93} & \asbar{100} & \asbar{99} & \asbar{93} & \asbar{93} & \asbar{100} & \asbar{99} \\ 
\cmidrule{2-10}
& \citealt{kim-linzen-2020-cogs} & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{30} & \asbar{45} & \asbar{35} \\
%& \citealt{ontanon-etal-2021-making} & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{51} & \asbar{43} & \asbar{56} & \asbar{48} \\ % table : rel2-eb-c small-6s seq2seq (not the strongest seq model, but strongest with per gen type results)
& \citealt{akyurek-andreas-2021-lexicon} & train & \asbar{0} & \asbar{0} & \asbar{1} & \asbar{66} & \asbar{64} & \asbar{100} & \asbar{82} \\
& \citealt{orhan-2021-compgen} & train & \asbar{0} & \asbar{0} & \asbar{10} & \asbar{84} & \asbar{86} & \asbar{100} & \asbar{85} \\
& \citealt{zheng-lapata-2021-disentangled} & train & \asbar{0} & \asbar{12} & \asbar{39} & \asbar{92} & \asbar{91} & \asbar{100} & \asbar{89} \\
& \citealt{kim-linzen-2020-cogs} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{23} & \asbar{54} & \asbar{77} & \asbar{63} \\
& \citealt{conklin-etal-2021-meta} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{20} & \asbar{66} & \asbar{94} & \asbar{75} \\
& \citealt{csordas-etal-2021-devil} & train100 & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{55} & \asbar{62} & \asbar{92} & \asbar{75} \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{syn}}} & BART & train100 & \asbar{1} & \asbar{4} & \asbar{8} & \asbar{97} & \asbar{94} & \asbar{96} & \asbar{83} \\
&T5 & train & \asbar{0} & \asbar{1} & \asbar{0} & \asbar{96} & \asbar{93} & \asbar{100} & \asbar{85} \\ 
% \cmidrule{2-10}
&T5+aug & train & \asbar{100} & \asbar{1} & \asbar{0} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
&T5+aug+close brackets & train & \asbar{100} & \asbar{69} & \asbar{10} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
& Benepar & train100 & \asbar{84} & \asbar{95} & \asbar{98} & \asbar{99} & \asbar{100} & \asbar{100} & \asbar{99} \\
\midrule
\parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{pos}}} & BART & train & \asbar{0} & \asbar{5} & \asbar{21} & \asbar{84} & \asbar{85} & \asbar{100} & \asbar{85} \\
& T5 & train & \asbar{0} & \asbar{0} & \asbar{0} & \asbar{73} & \asbar{78} & \asbar{100} & \asbar{83} \\
& T5+aug & train & \asbar{92} & \asbar{86} & \asbar{27} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{95} \\
% \midrule
% \parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{qa 1}}} & BART & train & \asbar{100} & \asbar{95} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
% \midrule
% \parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{qa 2}}} & BART & train & \asbar{68} & \asbar{53} & \asbar{63} & \asbar{63} & \asbar{89} & \asbar{100} & \asbar{86} \\
% & BART-QA & train & \asbar{90} & \asbar{68} & \asbar{100} & \asbar{86} & \asbar{91} & \asbar{100} & \asbar{94} \\
% \midrule
% \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{qa 3}}} & BART & train & \asbar{100} & \asbar{57} & \asbar{66} & \asbar{63} & \asbar{100} & \asbar{100} & \asbar{85} \\
% &T5 & train & \asbar{97} & \asbar{65} & \asbar{60} & \asbar{98} & \asbar{100} & \asbar{100} & \asbar{90} \\ 
% & BART-QA & train & \asbar{100} & \asbar{96} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{100} & \asbar{99} \\
\bottomrule
\end{tabular} 
    \caption{Exact match accuracies on the individual generalization types. We have compressed all 16 generalization types of the \lexg class into a single column and report the average accuracy. \todo{This table now need results from more seq2seq models like T5. Also now most results are based on train set rather than train100 so I need to run some BART experiments again. } \todo{Now the results in table 1 and table 2 are separate. I am also considering to merge them in one table but do not have a good idea on how to introduce them in the writing. }
    % \pw{to yuekun:}\yy{any updates from Z\&L re: per gen type results?}
    %Additionally to our own runs we copy numbers from \citet[Lex:Simple]{akyurek-andreas-2021-lexicon},  \citet[mT5 xl]{orhan-2021-compgen} and run own train100 experiments \yy{(1 run)} for \citet[\yy{model  config?}]{conklin-etal-2021-meta} and \citet[\yy{model  config?}]{csordas-etal-2021-devil}.
    }\label{tab:selected_gentype_eval}%\label{tab:selected_gentype_eval_transposed}
  \end{table*}

  
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/cogs_detailed_results.tex <==
\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll|ccc|c|c}
    \toprule
    & & \multicolumn{3}{c|}{\structg} & \lexg &   \\
    Dataset & Model & Obj to Subj PP & CP recursion & PP recursion & all 18 other types & overall \\
    \midrule
    \multirow{5}{*}{COGS} & BART & $0.0 \pm 0.0$ & $0.5 \pm 0.2$ & $11.8 \pm 1.5$ & $91.1 \pm 0.4$ & $78.6 \pm 0.3$ \\
    & BART+syn & $0.0 \pm 0.0$ & $5.3 \pm 0.8$ & $7.7 \pm 0.3$ & $92.8 \pm 0.5$ & $80.1 \pm 0.5$ \\
    & BART+mtl & $0.0 \pm 0.0$ & $0.3 \pm 0.2$ & $10.9 \pm 1.9$ & $92.1 \pm 0.3$ & $79.5 \pm 0.3$ \\
    & BART+mask & $0.0 \pm 0.0$ & $0.1 \pm 0.1$ & $4.9 \pm 2.9$ & $84.0 \pm 2.8$ & $72.2 \pm 2.5$ \\
    & T5 & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $8.6 \pm 2.2$ & $96.9 \pm 0.3$ & $83.5 \pm 0.2$ \\
    \midrule
    \multirow{2}{*}{Syntax-COGS} & BART & $0.0 \pm 0.0$ & $9.1 \pm 1.5$ & $22.3 \pm 1.1$ & $99.5 \pm 0.1$ & $86.8 \pm 0.1$ \\
    & T5 & $4.7 \pm 8.7$ & $7.2 \pm 1.3$ & $9.0 \pm 4.0$ & $99.4 \pm 0.5$ & $86.2 \pm 0.3$ \\
    \midrule
    \multirow{2}{*}{POS-COGS} & BART & $0.0 \pm 0.0$ & $5.8 \pm 5.2$ & $19.1 \pm 10.2$ & $97.9 \pm 1.0$ & $85.1 \pm 1.1$ \\
    & T5 & $0.0 \pm 0.0$ & $4.2 \pm 2.5$ & $3.9 \pm 4.1$ & $98.1 \pm 1.1$ & $84.5 \pm 0.9$ \\
    \midrule
    \multirow{3}{*}{QA-COGS-base} & BART & $98.9 \pm 0.7$ & $58.8 \pm 4.3$ & $69.1 \pm 1.0$ & $95.3 \pm 0.3$ & $85.7 \pm 0.7$ \\
    & T5 & $100.0 \pm 0.0$ & $94.7 \pm 2.3$ & $96.9 \pm 0.6$ & $100.0 \pm 0.0$ & $98.6 \pm 0.5$ \\
    & BART-QA & $100.0 \pm 0.0$ & $97.6 \pm 0.9$ & $99.6 \pm 1.0$ & $100.0 \pm 0.0$ & $99.2 \pm 0.4$ \\
    \midrule
    \multirow{4}{*}{\textit{cc\_cp}} & BART & - & - & - & - & $36.5 \pm 22.0$ \\
    & T5 & - & - & - & - & $15.6 \pm 1.7$ \\
    & BART-QA  & - & - & - & - & $5.6 \pm 10.0$ \\
    & BART-QA+struct  & - & - & - & - & $100.0 \pm 0.0$ \\ 
    \midrule
    \multirow{4}{*}{\textit{rc\_pp}} & BART & - & - & - & - & $13.7 \pm 5.1$ \\
    & T5 & - & - & - & - & $21.9 \pm 2.0$ \\
    & BART-QA  & - & - & - & - & $0.0 \pm 0.0$ \\
    & BART-QA+struct  & - & - & - & - & $100.0 \pm 0.0$ \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Detailed results for our models across COGS, Syntax-COGS, POS-COGS and QA-COGS.}
    \label{tab:detailed_results}
\end{table*}

==> tables/coordination_cp_example.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}


% \begin{table*}[]
%     \small
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{\linewidth}{X|X|X|X|X} \toprule
%         \multirow{2}{*}{Gen Type}& \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Generalization}} \\
%         % \hline
%         & \multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Question}}  & \multicolumn{1}{c}{\textbf{Context}} & \multicolumn{1}{c}{\textbf{Question}} \\
%         \hline
%         \multirow{3}{3.5cm}{\textit{cc\_cp}} & {Oliver liked that Noah discovers a boy } & {What did Oliver like?} & \multirow{3}{3cm}{Oliver liked that Noah discovers a boy and jogged . } & \multirow{3}{*}{What did Oliver like?} \\
%         & {Oliver slept and jogged} & {Who jogged?} & & \\
%         & {Oliver sleeps and jogs} & {Who jogs?} & & \\
%         \hline
%         \multirow{2}{3.5cm}{\textit{rc\_pp}} & {Olivia gave a box that was sketched to Benjamin} & { What was sketched?} & \multirow{2}{3cm}{Olivia gave a box in the houses that were sketched to Benjamin} & \multirow{2}{*}{What was sketched?} \\
%         & {Olivia gave boxes that were sketched to Benjamin} & {What was sketched?} & & \\
%          \bottomrule
%     \end{tabularx}
%     \caption{
%         Examples for our new generalization types. \textit{cc\_cp} denotes that we have complement clause and coordination structure separately during training and test their combination during generalization. \textit{rc\_pp} denotes that we have relative clause and preposition phrase structure separately during training and test their combination during generalization. 
%         % An example for combination of coordination structure and complement clause.
%         % \textcolor{red}{I reconsidered the \textit{cc\_cp} type and now I think the question we should ask in the test case is \textit{Who jogged?} rather than \textit{What did Oliver like?} }
%         % bold? underline? colors?
%     }\label{tab:coordination_cp_example}
% \end{table*}



==> tables/dataset_statistics.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{lccccccc}
    \toprule
    Dataset & \# train & \# dev. & \# test & \# gen & Vocab. size & Train len. & Gen len. \\
    \midrule
    COGS & 24155 & 3000 & 3000 & 21000 & 871 & $22 / 153$ & $61 / 480$ \\
    \midrule
    Syntax-COGS & 24155 & 3000 & 3000 & 21000 & 759 & $22 / 129$ & $61 / 375$ \\
    \midrule
    POS-COGS & 24155 & 3000 & 3000 & 21000 & 753 & $22 / 21$ & $61 / 60$ \\
    \midrule
    QA-COGS-base & 54349 & 6834 & 6798 & 67989 & 793 & $44 / 19$ & $123 / 57$ \\
    \midrule
    \multirow{4}{*}{\textit{cc\_cp} (4 splits)} & 4000 & 1000 & 1000 & 2000 & 709 & $36 / 25$ & $35 / 18$ \\
     & 4000 & 1000 & 1000 & 2000 & 709 & $35 / 21$ & $36 / 25$ \\
     & 4000 & 1000 & 1000 & 2000 & 709 & $36 / 25$ & $30 / 19$ \\
     & 4000 & 1000 & 1000 & 2000 & 709 & $36 / 25$ & $34 / 21$ \\
     \midrule
    \multirow{4}{*}{\textit{rc\_pp} (4 splits)} & 4000 & 1000 & 1000 & 2000 & 594 & $19 / 5$ & $19 / 5$ \\
     & 4000 & 1000 & 1000 & 2000 & 594 & $19 / 5$ & $19 / 2$ \\
     & 4000 & 1000 & 1000 & 2000 & 594 & $19 / 5$ & $19 / 2$ \\
     & 4000 & 1000 & 1000 & 2000 & 594 & $19 / 5$ & $19 / 5$ \\
    \bottomrule
    \end{tabular}
    \caption{Statistics for all our datasets. \# denotes the number of instances in the dataset. Vocab.size denotes the size of vocabulary for the dataset, which consists of input tokens and output tokens. Train.len denotes the maximum length of the input tokens and output tokens in the train set. Gen.len denotes the maximum length in the generalization set.}
    \label{tab:dataset_statistics}
\end{table*}

==> tables/obj_to_subj_pp_error.tex <==
% \begin{figure}
%     \centering
%     \begin{tabularx}{\linewidth}{l|X}
%         \toprule
%          {Input} & {The cake on the table burned.}  \\
%          \midrule
%          {Sem} & \footnotesize {\lform{*cake($x_1$); *table($x_4$); cake.nmod.on($x_1,x_4$) $\land$ burn.theme($x_3, x_1$)}} \\
%          \midrule
%          {T5} & \footnotesize{\lform{*cake($x_1$); *table($x_7$); burn.theme($x_2, x_1$) $\land$ burn.theme($x_2, x_4$)}} \\
%          \midrule
%          {Syn} & \footnotesize{\lform{( S ( VP ( NP ( Det The ) ( N cake ) ( PP ( P on ) ( NP ( Det the ) ( N table ) ) ) ) ( V burned ) ) )}} \\
%          \midrule
%          {T5} & \footnotesize{\lform{( S ( VP ( NP ( Det The ) ( N cake ) ( VP ( V on ) ( NP ( Det the ) ( N table ) ) ) ))}} \\
%          \midrule
%          {POS} & \footnotesize{\lform{Det N P Det N V }} \\
%          \midrule
%          {T5} & \footnotesize{\lform{Det N V Det N P Det N}} \\
%          \bottomrule
%     \end{tabularx} 
%     \caption{Example for \textit{obj\_to\_subj\_pp} type. We list the annotation of semantic parse, syntax tree and POS tags with corresponding T5 predictions. }
%     \label{fig:error_example}
% \end{figure}


\begin{figure}
    \centering
    \scriptsize
    \begin{tabular}{@{}llm{.7\linewidth}@{}}
        \toprule
         &  {Input} & {The baby on a tray in the house screamed.}  \\
         \midrule
         \multirow{2}{*}{ \rotatebox[origin=c]{90}{Semantics\quad}} &  {Gold} &  {\lform{*baby($x_1$); *house($x_7$); baby.nmod.on($x_1$,$x_4$) $\land$ tray($x_4$) $\land$ tray.nmod.in($x_4$,$x_7$) $\land$ scream.agent($x_8$,$x_1$) }} \\
         \cmidrule(l){2-3}
         &  {T5} &  {\lform{*baby($x_1$); *house(\textcolor{red}{$x_{10}$}); \textcolor{red}{scream.agent($x_2$,$x_1$)} $\land$ \textcolor{red}{scream.theme($x_2$,$x_4$)} $\land$ tray($x_4$) $\land$ tray.nmod.in($x_4$,$x_7$)}} \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{Syntax\quad\quad}} &  {Gold} & {\lform{( S ( NP ( Det The ) ( N baby ) ( PP ( P on ) ( NP ( Det a ) ( N tray ) ( PP ( P in ) ( NP ( Det the ) ( N house ) ) ) ) ) ) ( VP ( V screamed ) ) ) }} \\
         \cmidrule(l){2-3}
         &  {T5} & {\lform{( S ( NP ( Det The ) ( N baby ) ( \textcolor{red}{VP} ( \textcolor{red}{V} on ) ( NP ( Det a ) ( N tray ) ( PP ( P in ) ( NP ( Det the ) ( N house ) ) ) ) ) ) \textcolor{red}{)}}} \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{POS\;\;}} &  {Gold} & {\lform{Det N P Det N P Det N V}} \\
         \cmidrule(l){2-3}
         &   {T5} & {\lform{Det N \textcolor{red}{V} Det N P Det N \textcolor{red}{P Det N}}} \\
         \bottomrule
    \end{tabular} 
    \caption{Example for \textit{obj\_to\_subj\_pp} type. We list the annotation of semantic parse, syntax tree and POS tags with corresponding T5 predictions. }
    \label{fig:error_example}
\end{figure}

==> tables/qa_detailed_results.tex <==
\begin{table}[]
    \small
    \centering
\begin{tabular}{lcc}
Type & BART & BART-QA \\ \midrule
Subj to Obj (common noun) & 100 & 100\\
Subj to Obj (proper noun) & 100 & 100 \\
Obj to Subj (common noun) & 100  & 100 \\
Obj to Subj (proper noun) & 100 & 100  \\ 
\midrule
Prim to Subj (common noun) & 100 & 100 \\
Prim to Subj (proper noun) & 96 & 100 \\
Prim to Obj (common noun) & 100 & 100 \\
Prim to Obj (proper noun) & 63 & 100 \\
Prim verb to Infin. arg & 55 & 100 \\
\midrule
ObjmodPP to SubjmodPP & 100 & 100 \\
CP recursion & 57 & 96  \\
PP recursion & 66 & 100 \\
\midrule
Active to Passive & 100 & 100 \\
Passive to Active & 100 & 100 \\
ObjOTrans. to trans. & 100 & 100 \\
Unacc to transitive & 100 & 100 \\
Dobj dative to PP dative & 100 & 100 \\
PP dative to Dobj dative & 100 & 100 \\ 
\midrule
Agent NP to Unacc Subj & 100  & 100\\
Theme NP to ObjOTrans. Subj & 100 & 100 \\
Theme NP to Unergative Subj & 100 & 100 \\ 
\midrule
Total & 85 & 99\\
\bottomrule
    \end{tabular}
    \caption{
        Exact match accuracy on the generalization set by generalization type
        \todo{We may need more columns for T5, LSTM and transformers (without pretraining). In that case, maybe it's better to changed this table into the format we used in the reject paper?}
    }\label{tab:qa_detailed_results}
\end{table}

==> tables/qa_prim_error_examples.tex <==
\begin{table*}[htb!]
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{\linewidth}{l|X|X|X|X} \toprule
         \textbf{generalization types} & \textbf{Context} & \textbf{Question} & \textbf{Gold} & Pred\\ 
         \midrule
         \textit{prim\_to\_subj\_proper} & {Noah imagined that Emma supported that Paula wanted to dance .}  & {Who did Noah imagine that Emma support that want to dance ?} & {Paula} & {Paula Paula}\\
         \midrule
        \textit{prim\_to\_obj\_proper} & {Evelyn gave Paula to a journalist .} & {What did Evelyn give to a journalist ?} & {Paula} & {Paula Paula} \\
        \midrule
        \textit{prim\_to\_inf\_arg} & {The consumer hated to crawl .} & {What did the consumer hate to do ?} & {crawl} & {crawl crawl} \\
        % \midrule
        % \textit{obj\_pp\_to\_subj\_pp} & {The baby on a tray in the house screamed .} & {Who screamed ?} & {the baby on a tray in the house} & {the baby on a tray in the house} \\
         \bottomrule
    \end{tabularx}
    \caption{
        Some examples for the QA-COGS dataset.
        % bold? underline? colors?
    }\label{tab:qa_prim_error_examples}
\end{table*}

==> tables/rc_example.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{lXX} \toprule
Context & \textit{Emma ate the rings beside a bed that \textcolor{red}{was} called} & \textit{Emma ate the rings beside a bed that \textcolor{red}{were} called} \\
\midrule
Gold &  \textit{a bed} & \textit{the rings beside a bed}\\
BART &  \textit{the rings beside a bed} & \textit{the rings beside a bed} \\
BART-QA &  \textit{the rings beside a bed} & \textit{the rings beside a bed} \\
 \bottomrule
\end{tabularx}
\caption{Error example for BART and BART-QA. In this sentence the question is \textit{What was called?}}\label{tab:error_rc}
\end{table}


==> tables/struct_gen_type_results.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}{ccccccccccc}
%     \multirow{2}{*}{ Model } & \multicolumn{5}{c}{rc\_pp} & \multicolumn{5}{c}{cc\_cp} \\
%     & sg\_pl & sg\_sg & pl\_sg & pl\_pl & avg & ps\_pr & ps\_ps & pr\_ps & pr\_pr & avg \\
%     BART & 14 & 80 & 2 & 96 & 48 & 1 & 100 & 1 & 100 & 51 \\
%     BART-QA & 6 & 85 & 0 & 100 & 48 & 48 & 74 & 62 & 85 & 67 \\    \end{tabular}
%     \caption{exact accuracy on new test set }
%     \todo{I plan to change the coordination experiments so will update this table after that. }

%     \label{tab:qa_struct_results}
% \end{table*}

\begin{table}[]
    \centering
    \begin{tabular}{c|cc}
    Model & rc\_pp & cc\_cp \\
    \toprule
    BART & 48 & 51 \\
    BART-QA & 48 & 67 \\
    BART-QA+syn & - & 100 \\
    \bottomrule
    \end{tabular}
    \caption{exact accuracy on new test set }
    % \todo{I plan to change the coordination experiments so will update this table after that. }

    \label{tab:qa_struct_results}
\end{table}
